A Benchmark for Semi-Inductive Link Prediction in Knowledge Graphs

Semi-inductive link prediction (LP) in knowledge graphs (KG) is the task of predicting facts for new, previously unseen entities based on context information. Although new entities can be integrated by retraining the model from scratch in principle, such an approach is infeasible for large-scale KGs, where retraining is expensive and new entities may arise frequently. In this paper, we propose and describe a large-scale benchmark to evaluate semi-inductive LP models. The benchmark is based on and extends Wikidata5M: It provides transductive, k-shot, and 0-shot LP tasks, each varying the available information from (i) only KG structure, to (ii) including textual mentions, and (iii) detailed descriptions of the entities. We report on a small study of recent approaches and found that semi-inductive LP performance is far from transductive performance on long-tail entities throughout all experiments. The benchmark provides a test bed for further research into integrating context and textual information in semi-inductive LP models.

==> emnlp2023/small-macros.tex <==
% File: macros.tex
%
% Contains general macros for use with LaTeX.
%
% $LastChangedRevision: 961 $
% $LastChangedDate: 2008-08-25 18:43:18 +0200 (Mon, 25 Aug 2008) $
%
% Author: Rainer Gemulla
%
% Packages:
% \usepackage{array}
% \usepackage{amsxtra}



% this is just the default macros file with some commented out



% --------------
% EDITING MACROS
% --------------
%\newcommand{\todo}[1]{\textcolor{red}{#1}} % todos
\newcommand{\co}[1]{\textcolor{blue}{#1}} % comments
\newcommand{\eat}[1]{} % TO MAKE LARGE BLOCKS OF TEXT INVISIBLE

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\dgreen}[1]{\textcolor{green!70!black}{#1}}
\newcommand{\orange}[1]{\textcolor{orange}{#1}}
\newcommand{\yellow}[1]{\textcolor[rgb]{102, 77, 0}{#1}}

% -------------
% CARDINALITIES
% -------------
\newcommand{\sz}[1]{\lvert#1\rvert}   % cardinality of set
\newcommand{\card}[1]{\lvert#1\rvert} % cardinality of set
\newcommand{\Sz}[1]{\lVert#1\rVert}   % cardinality of set, distinct (not used in thesis!)
\newcommand{\Card}[1]{\lVert#1\rVert} % cardinality of set, distinct (not used in thesis!)

% ----------
% EQUALITIES
% ----------
\newcommand{\eqdef}{\stackrel{\mathrm{def}}{=}} % definining equality
\newcommand{\eqdot}{\doteq} % APPROACHES THE LIMIT (asymptotic equality)
\newcommand{\eqdist}{\equiv} % equality in distribution

% --------
% ROUNDING
% --------
\newcommand{\floor}[1]{\left\lfloor#1\right\rfloor} % floor, automatic brackets
\newcommand{\floorn}[1]{\lfloor#1\rfloor} % floor, normal brackets
\newcommand{\ceil}[1]{\left\lceil#1\right\rceil} % ceil, automatic brackets
\newcommand{\ceiln}[1]{\lceil#1\rceil} % ceil, normal brackets

% ---------------
% ABSOLUTE VALUES
% ---------------
\newcommand{\abs}[1]{\left\lvert#1\right\rvert} % abs, automatic brackets
\newcommand{\absn}[1]{\lvert#1\rvert} % abs, normal brackets

% ---------------------
% SUPER- AND SUBSCRIPTS
% ---------------------
\newcommand{\td}[2]{\if*#1\else^{#1}\fi\if*#2\else_{#2}\fi} % ^?_?, *=ignore

% -----------
% PROBABILITY
% -----------
\newcommand{\xpr}[2]{p\td{#1}{#2}} % Pr^?_?
\newcommand{\uxpr}[2]{\tilde p\td{#1}{#2}} % ~Pr^?_?
\newcommand{\pr}[1]{\xpr**\!\left(#1\right)} % Pr(?], automatic brackets
\newcommand{\prn}[1]{\xpr**\!(#1)} % Pr(?], normal brackets
\newcommand{\prbig}[1]{\xpr**\!\bigl(#1\bigr)} % Pr(?], big brackets
\newcommand{\prBig}[1]{\xpr**\!\Bigl(#1\Bigr)} % Pr(?], Big brackets
\newcommand{\prbigg}[1]{\xpr**\!\biggl(#1\biggr)} % Pr(?], bigg brackets
\newcommand{\prBigg}[1]{\xpr**\!\Biggl(#1\Biggr)} % Pr(?], Bigg brackets

\newcommand{\prf}[3]{\xpr{#1}{#2}\!\left(#3\right)} % Pr^?_?(?), automatic brackets
\newcommand{\uprf}[3]{\uxpr{#1}{#2}\!\left(#3\right)} % ~Pr^?_?(?), automatic brackets

\newcommand{\prs}[1]{\xpr**\!\left(#1\right)} % Pr(?], automatic brackets, no spacing
\newcommand{\prsn}[1]{\xpr**\!(#1)} % Pr(?], normal brackets, no spacing

\newcommand{\Pa}{\operatorname{Pa}}
\newcommand{\Nd}{\operatorname{NonDescendants}}

% -------------
% SPACING
% -------------
\newcommand\macrospace{}

% --------------
% EXPECTED VALUE
% --------------
\newcommand{\xev}[2]{\operatorname{E}\td{#1}{#2}} % E^?_?

\newcommand{\evf}[3]{\xev{#1}{#2}{\left[\macrospace{}#3\macrospace{}\right]}} % E^?_?[?], automatic brackets
\newcommand{\evfn}[3]{\xev{#1}{#2}{[\macrospace{}#3\macrospace{}]}} % E^?_?[?], normal brackets
\newcommand{\evfbig}[3]{\xev{#1}{#2}{\bigl[\macrospace{}#3\macrospace{}\bigr]}} % E^?_?[?], big brackets
\newcommand{\evfBig}[3]{\xev{#1}{#2}{\Bigl[\macrospace{}#3\macrospace{}\Bigr]}} % E^?_?[?], Big brackets
\newcommand{\evfbigg}[3]{\xev{#1}{#2}{\biggl[\macrospace{}#3\macrospace{}\biggr]}} % E^?_?[?], bigg brackets

\newcommand{\ev}[1]{\evf**{#1}} % E[?], automatic brackets
\newcommand{\evn}[1]{\evfn**{#1}} % E[?], normal brackets
\newcommand{\evbig}[1]{\evfbig**{#1}} % E[?], big brackets
\newcommand{\evBig}[1]{\evfBig**{#1}} % E[?], Big brackets
\newcommand{\evbigg}[1]{\evfbigg**{#1}} % E[?], bigg brackets

% ----
% BIAS
% ----
\newcommand{\xbias}[2]{\operatorname{bias}\td{#1}{#2}} % Bias^?_?
\newcommand{\bias}[1]{\xbias**\left[\macrospace{}#1\macrospace{}\right]} % Bias[?], automatic brackets
\newcommand{\biasn}[1]{\xbias**[\macrospace{}#1\macrospace{}]} % Bias[?], normal brackets

% --------
% VARIANCE
% --------
\newcommand{\xvar}[2]{\operatorname{var}\td{#1}{#2}} % Var^?_?
\newcommand{\var}[1]{\xvar**\left[\macrospace{}#1\macrospace{}\right]} % Var[?], automatic brackets
\newcommand{\varn}[1]{\xvar**[\macrospace{}#1\macrospace{}]} % Var[?], normal brackets
\newcommand{\varbig}[1]{\xvar**\bigl[\macrospace{}#1\macrospace{}\bigr]} % Var[?], big brackets
\newcommand{\varBig}[1]{\xvar**\Bigl[\macrospace{}#1\macrospace{}\Bigr]} % Var[?], Big brackets

\newcommand{\xhatvar}[2]{\operatorname{\hat{v}ar}\td{#1}{#2}} % ~Var^?_?
\newcommand{\hatvar}[1]{\xhatvar**\left[\macrospace{}#1\macrospace{}\right]} % ~Var[?], automatic brackets
\newcommand{\hatvarn}[1]{\xhatvar**[\macrospace{}#1\macrospace{}]} % ~Var[?], normal brackets
\newcommand{\hatvarBig}[1]{\xhatvar**\Bigl[\macrospace{}#1\macrospace{}\Bigr]} % ~Var[?], Big brackets

\newcommand{\varf}[3]{\xvar{#1}{#2}{\left[\macrospace{}#3\macrospace{}\right]}} % Var^?_?[?], automatic brackets
\newcommand{\varfn}[3]{\xvar{#1}{#2}{[\macrospace{}#3\macrospace{}]}} % E^?_?[?], normal brackets
\newcommand{\varfbig}[3]{\xvar{#1}{#2}{\bigl[\macrospace{}#3\macrospace{}\bigr]}} % E^?_?[?], big brackets
\newcommand{\varfBig}[3]{\xvar{#1}{#2}{\Bigl[\macrospace{}#3\macrospace{}\Bigr]}} % E^?_?[?], Big brackets
\newcommand{\varfbigg}[3]{\xvar{#1}{#2}{\biggl[\macrospace{}#3\macrospace{}\biggr]}} % E^?_?[?], bigg

% ----------
% COVARIANCE
% ----------
\newcommand{\xcov}[2]{\operatorname{Cov}\td{#1}{#2}} % Cov^?_?
\newcommand{\cov}[1]{\xcov**\left[\macrospace{}#1\macrospace{}\right]} % Cov[?], automatic brackets
\newcommand{\covn}[1]{\xcov**[\macrospace{}#1\macrospace{}]} % Cov[?], normal brackets
\newcommand{\covBig}[1]{\xcov**\Bigl[\macrospace{}#1\macrospace{}\Bigr]} % Cov[?], Big brackets

\newcommand{\xhatcov}[2]{\operatorname{\hat{C}ov}\td{#1}{#2}} % ~Cov^?_?
\newcommand{\hatcov}[1]{\xhatcov**\left[\macrospace{}#1\macrospace{}\right]} % ~Cov[?], automatic brackets
\newcommand{\hatcovn}[1]{\xhatcov**[\macrospace{}#1\macrospace{}]} % ~Cov[?], normal brackets
\newcommand{\hatcovBig}[1]{\xhatcov**\Bigl[\macrospace{}#1\macrospace{}\Bigr]} % ~Cov[?], Big brackets

% --------------
% STANDARD ERROR
% --------------

\newcommand{\xse}[2]{\operatorname{SE}\td{#1}{#2}} % SE^?_?
\newcommand{\se}[1]{\xse**\left[\macrospace{}#1\macrospace{}\right]} % SE[?], automatic brackets
\newcommand{\sen}[1]{\xse**[\macrospace{}#1\macrospace{}]} % SE[?], normal brackets

\newcommand{\xhatse}[2]{\operatorname{\hat{S}E}\td{#1}{#2}} % ~SE^?_?
\newcommand{\hatse}[1]{\xhatse**\left[\macrospace{}#1\macrospace{}\right]} % ~SE[?], automatic brackets
\newcommand{\hatsen}[1]{\xhatse**[\macrospace{}#1\macrospace{}]} % ~SE[?], normal brackets

% --------------
% STANDARD ERROR
% --------------

\newcommand{\xsd}[2]{\operatorname{SD}\td{#1}{#2}} % SD^?_?
\newcommand{\sd}[1]{\xsd**\left[\macrospace{}#1\macrospace{}\right]} % SD[?], automatic brackets
\newcommand{\sdn}[1]{\xsd**[\macrospace{}#1\macrospace{}]} % SD[?], normal brackets

\newcommand{\xhatsd}[2]{\operatorname{\hat{S}D}\td{#1}{#2}} % ~SD^?_?
\newcommand{\hatsd}[1]{\xhatsd**\left[\macrospace{}#1\macrospace{}\right]} % ~SD[?], automatic brackets
\newcommand{\hatsed}[1]{\xhatsd**[\macrospace{}#1\macrospace{}]} % ~SD[?], normal brackets


% ------------------------
% COEFFICIENT OF VARIATION
% ------------------------
\newcommand{\xcv}[2]{\operatorname{CV}\td{#1}{#2}} % Cv^?_?
\newcommand{\cv}[1]{\xcv**\left[\macrospace{}#1\macrospace{}\right]} % Cv[?], automatic brackets
\newcommand{\cvn}[1]{\xcv**[\macrospace{}#1\macrospace{}]} % Var[?], normal brackets
\newcommand{\cvbig}[1]{\xcv**\bigl[\macrospace{}#1\macrospace{}\bigr]} % Cv[?], big brackets
\newcommand{\cvBig}[1]{\xcv**\Bigl[\macrospace{}#1\macrospace{}\Bigr]} % Cv[?], Big brackets

% -----------------
% MEAN SQUARE ERROR
% -----------------
\newcommand{\xmse}[2]{\operatorname{mse}\td{#1}{#2}} % MSE^?_?
\newcommand{\mse}[1]{\xmse**\left[\macrospace{}#1\macrospace{}\right]} % MSE[?], automatic brackets
\newcommand{\msen}[1]{\xmse**[\macrospace{}#1\macrospace{}]} % MSE[?], normal brackets

% ----------------------
% ROOT MEAN SQUARE ERROR
% ----------------------
\newcommand{\xrmse}[2]{\operatorname{rmse}\td{#1}{#2}} % RMSE^?_?
\newcommand{\rmse}[1]{\xrmse**\left[\macrospace{}#1\macrospace{}\right]} % RMSE[?], automatic brackets
\newcommand{\rmsen}[1]{\xrmse**[\macrospace{}#1\macrospace{}]} % RMSE[?], normal brackets

% ----------------------
% AVERAGE RELATIVE ERROR
% ----------------------
\newcommand{\xare}[2]{\operatorname{ARE}\td{#1}{#2}} % ARE^?_?
\newcommand{\are}[1]{\xare**\left[\macrospace{}#1\macrospace{}\right]} % ARE[?], automatic brackets
\newcommand{\aren}[1]{\xare**[\macrospace{}#1\macrospace{}]} % ARE[?], normal brackets

% ---------------------
% BINOMIAL DISTRIBUTION
% ---------------------

% B(k; N,q)
\newcommand{\pbinom}[3]{B\!\left(#1;\,#2,#3\right)} % binomial probability, automatic brackets

% ---------------------------
% HYPERGEOMETRIC DISTRIBUTION
% ---------------------------
\newcommand{\phyper}[4]{H\!\left(#1;\,#2,#3,#4\right)} % hypergeometric probability, automatic brackets

% --------------
% ARGMIN, ARGMAX
% --------------
%\DeclareMathOperator*{\argmin}{argmin} % amsmath package required
%\DeclareMathOperator*{\argmax}{argmax} % amsmath package required

% ----
% SETS
% ----
\renewcommand\:{\colon} % for use with \sset, etc.
\newcommand{\sset}[1]{\left\{\,#1\,\right\}} % { ? }, automatic brackets
\newcommand{\ssets}[1]{\left\{#1\right\}} % {?}, automatic brackets
\newcommand{\ssetn}[1]{\{\,#1\,\}} % { ? }, normal brackets

\newcommand{\comp}[1]{\bar{#1}} % complement

\newcommand{\powerset}[1]{\cP\!\left(#1\right)} % powerset, automatic brackets

\newcommand\adots{{\ensuremath ..}} % short array notation as in A[i..j]

\newcommand{\Nat}{{\ensuremath \bN}}
\newcommand{\Bool}{{\ensuremath \{0,1\}}}

% --------
% BOOLEANS
% --------
\newcommand\true{\text{true}} % use in math mode
\newcommand\false{\text{false}} % use in math mode

% --------------------
% RELATIONAL OPERATORS
% --------------------
\newcommand\join\Join % normal join

% uses txfonts for left/right semi join symbols (and nothing else)
\DeclareSymbolFont{txsymbolsC}{U}{txsyc}{m}{n}
\SetSymbolFont{txsymbolsC}{bold}{U}{txsyc}{bx}{n}
\DeclareFontSubstitution{U}{txsyc}{m}{n}
\DeclareMathSymbol{\ljoin}{\mathrel}{txsymbolsC}{88}
\DeclareMathSymbol{\rjoin}{\mathrel}{txsymbolsC}{89}
%\DeclareMathSymbol{\join}{\mathrel}{txsymbolsC}{90} NOT NEEDED

% -----------
% SQL queries
% -----------
\newcommand{\sql}[1]{\texttt{#1}}

% -------------------
% MULTISET OPERATIONS
% -------------------
\newcommand\mcup{\uplus}       % multiset union
\newcommand\bigmcup{\biguplus} % multiset union, big
\newcommand\mcap{\nplus}       % multiset intersection
\newcommand\bigmcap{\nbigplus} % multiset intersection, big

\newsavebox\setminusbox
\newlength\setminuslen
\newcommand\msetminus{{\savebox{\setminusbox}{$\setminus$}\settowidth{\setminuslen}{\usebox{\setminusbox}}\,\usebox{\setminusbox}\hspace{-.5\setminuslen}^+}} % multiset difference
\newcommand\msetminusl{{\savebox{\setminusbox}{$_\setminus$}\settowidth{\setminuslen}{\usebox{\setminusbox}}\setminus\hspace{-.5\setminuslen}^+}} % multiset difference, when used as subscript


% -----------------
% MATRIX OPERATIONS
% -----------------
\newcommand\xdiag{\operatorname{diag}}
\newcommand\diag[1]{\xdiag\left(#1\right)}    % diagonal matrix
\newcommand\diagn[1]{\xdiag(#1)}    % diagonal matrix, normal brackets
\newcommand\xrank{\operatorname{rank}}
\newcommand\rank[1]{\xrank\left(#1\right)}
\newcommand\rankn[1]{\xrank(#1)}

% determinant: \det

\newcommand\T{\top}
\newcommand\transpose[1]{#1^{\T}}
\newcommand\tr[1]{#1^{\textrm{T}}}
%\newcommand\norm[1]{\left\lVert #1 \right\rVert}
\newcommand\normn[1]{\lVert #1 \rVert}
\newcommand\fnorm[1]{\left\lVert #1 \right\rVert_\text{F}}
\newcommand\fnormn[1]{\lVert #1 \rVert_\text{F}}
\newcommand\rsim{\stackrel{\mathrm{row}}{\sim}}
\newcommand\csim{\stackrel{\mathrm{col}}{\sim}}


% --------------------------
% TABULAR COLUMNS, MATH MODE
% --------------------------

\newcolumntype{C}{>{$\displaystyle}c<{$}} % centered math
\newcolumntype{L}{>{$\displaystyle}l<{$}} % left math
\newcolumntype{R}{>{$\displaystyle}r<{$}} % right math
\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}} % hide column

% extra spacing for math tables (used for after math rows set in display style if no rule follows)
\newcommand{\mathls}{\addlinespace[5pt]}

\newcommand{\mlsideways}[1]{\begin{sideways}\centering\begin{tabular}{c}#1\end{tabular}\end{sideways}} % multi-line sideways, centered

% ---------
% FUNCTIONS
% ---------
\newcommand{\func}[1]{\textsc{#1}} % function names for programming

% \newcommand{\G}[1]{\Gamma(#1)} % gamma function
\newcommand{\GQ}[2]{Q_{#1}(#2)} % regularized (upper) incomplete gamma function
\newcommand{\GP}[2]{P_{#1}(#2)} % regularized (lower) incomplete gamma function
\newcommand{\B}[3]{B\if*#1\else_{#1}\fi(#2,#3)} % (incomplete) beta function
\newcommand{\I}[3]{I\if*#1\else_{#1}\fi(#2,#3)} % regularized incomplete beta function
\newcommand{\Digamma}[1]{\Psi(#1)} % digamma function
\newcommand{\harmonic}[1]{H_{#1}} % harmonic number

% (mod ...), tight spacing
\makeatletter
\def\imod#1{\allowbreak\mkern10mu({\operator@font mod}\,\,#1)}
\makeatother

% ------
% BIG-OH
% ------
\newcommand{\bigO}[1]{O\!\left(#1\right)} % at most
\newcommand{\bigOn}[1]{O(#1)} % at most
\newcommand{\bigObig}[1]{O\bigl(#1\bigr)} % at most
\newcommand{\bigOmega}[1]{\Omega\!\left(#1\right)} % at least
\newcommand{\bigOmegan}[1]{\Omega(#1)} % at least
\newcommand{\bigTheta}[1]{\Theta\!\left(#1\right)} % at least and at most
\newcommand{\smallo}[1]{o\!\left(#1\right)} % asymptotically negligible (ratio f(x)/g(x)-->0)

%% -----------
%% CONVERGENCE
%% -----------
\newcommand{\toas}{\xrightarrow{\text{a.s.}}}

% -----------
% INTEGRATION
% -----------
\newcommand{\dd}{\; \mathrm{d}} % correct spacing and formating


% ------------
% ENVIRONMENTS
% ------------
%\newtheorem{lemma}{Lemma}
%\newtheorem{theorem}{Theorem}
%\newtheorem{proposition}{Proposition}
%\newtheorem{corollary}{Corollary}

% ------
% SPACES
% ------
\newlength\hspaceoflen
\newcommand\hspaceof[1]{\settowidth\hspaceoflen{#1}\hspace\hspaceoflen}

%% vertically centered
\newcommand{\vcentered}[1]{\begingroup\setbox0=\hbox{#1}\parbox{\wd0}{\box0}\endgroup}

% ----------------
% VECTOR VARIABLES
% ----------------
\newcommand\vect[1]{{\boldsymbol{#1}}}
\newcommand\va{\vect{a}}
\newcommand\vb{\vect{b}}
\newcommand\vc{\vect{c}}
\newcommand\vd{\vect{d}}
\newcommand\ve{\vect{e}}
\newcommand\vf{\vect{f}}
\newcommand\vg{\vect{g}}
\newcommand\vh{\vect{h}}
\newcommand\vi{\vect{i}}
\newcommand\vj{\vect{j}}
\newcommand\vk{\vect{k}}
\newcommand\vl{\vect{l}}
\newcommand\vm{\vect{m}}
\newcommand\vn{\vect{n}}
\newcommand\vo{\vect{o}}
\newcommand\vp{\vect{p}}
\newcommand\vq{\vect{q}}
\newcommand\vr{\vect{r}}
\newcommand\vs{\vect{s}}
\newcommand\vt{\vect{t}}
\newcommand\vu{\vect{u}}
\newcommand\vv{\vect{v}}
\newcommand\vw{\vect{w}}
\newcommand\vx{\vect{x}}
\newcommand\vy{\vect{y}}
\newcommand\vz{\vect{z}}
\newcommand\vzero{\vect{0}}
\newcommand\vone{\vect{1}}

\newcommand\valpha{\vect{\alpha}}
\newcommand\vbeta{\vect{\beta}}
\newcommand\veps{\vect{\epsilon}}
\newcommand\vdelta{\vect{\delta}}
\newcommand\veta{\vect{\eta}}
\newcommand\vgamma{\vect{\gamma}}
\newcommand\vtau{\vect{\tau}}
\newcommand\vtheta{\vect{\theta}}
\newcommand\vmu{\vect{\mu}}
\newcommand\vsigma{\vect{\sigma}}
\newcommand\vpi{\vect{\pi}}
\newcommand\vlambda{\vect{\lambda}}

% ----------------
% MATRIX VARIABLES
% ----------------
\newcommand\mA{\vect{A}}
\newcommand\mB{\vect{B}}
\newcommand\mC{\vect{C}}
\newcommand\mD{\vect{D}}
\newcommand\mE{\vect{E}}
\newcommand\mF{\vect{F}}
\newcommand\mG{\vect{G}}
\newcommand\mH{\vect{H}}
\newcommand\mI{\vect{I}}
\newcommand\mJ{\vect{J}}
\newcommand\mK{\vect{K}}
\newcommand\mL{\vect{L}}
\newcommand\mM{\vect{M}}
\newcommand\mN{\vect{N}}
\newcommand\mO{\vect{O}}
\newcommand\mP{\vect{P}}
\newcommand\mQ{\vect{Q}}
\newcommand\mR{\vect{R}}
\newcommand\mS{\vect{S}}
\newcommand\mT{\vect{T}}
\newcommand\mU{\vect{U}}
\newcommand\mV{\vect{V}}
\newcommand\mW{\vect{W}}
\newcommand\mX{\vect{X}}
\newcommand\mY{\vect{Y}}
\newcommand\mZ{\vect{Z}}
\newcommand\mzero{\vect{0}}

\newcommand{\mEps}{{\ensuremath{\vect{\Epsilon}}}}
\newcommand{\mSigma}{{\ensuremath{\vect{\Sigma}}}}
\newcommand{\mLambda}{{\ensuremath{\vect{\Lambda}}}}
\newcommand{\mPsi}{{\ensuremath{\vect{\Psi}}}}

% ------------------
% BLACKBOARD LETTERS
% ------------------
\newcommand\bA{\mathbb{A}}
\newcommand\bB{\mathbb{B}}
\newcommand\bC{\mathbb{C}} % set of complex numbers
\newcommand\bD{\mathbb{D}}
\newcommand\bE{\mathbb{E}}
\newcommand\bF{\mathbb{F}}
\newcommand\bG{\mathbb{G}}
\newcommand\bH{\mathbb{H}}
\newcommand\bI{\mathbb{I}}
\newcommand\bJ{\mathbb{J}}
\newcommand\bK{\mathbb{K}}
\newcommand\bL{\mathbb{L}}
\newcommand\bM{\mathbb{M}}
\newcommand\bN{\mathbb{N}} % set of positive integers
\newcommand\bO{\mathbb{O}}
\newcommand\bP{\mathbb{P}}
\newcommand\bQ{\mathbb{Q}} % set of rationals
\newcommand\bR{\mathbb{R}} % set of reals
\newcommand\bS{\mathbb{S}}
\newcommand\bT{\mathbb{T}}
\newcommand\bU{\mathbb{U}}
\newcommand\bV{\mathbb{V}}
\newcommand\bW{\mathbb{W}}
\newcommand\bX{\mathbb{X}}
\newcommand\bY{\mathbb{Y}}
\newcommand\bZ{\mathbb{Z}} % set of all integers

% -------------
% FANCY LETTERS
% -------------

% requires mathrsfs package
\newcommand\xA{\mathscr{A}}
\newcommand\xB{\mathscr{B}}
\newcommand\xC{\mathscr{C}}
\newcommand\xD{\mathscr{D}}
\newcommand\xE{\mathscr{E}}
\newcommand\xF{\mathscr{F}}
\newcommand\xG{\mathscr{G}}
\newcommand\xH{\mathscr{H}}
\newcommand\xI{\mathscr{I}}
\newcommand\xJ{\mathscr{J}}
\newcommand\xK{\mathscr{K}}
\newcommand\xL{\mathscr{L}}
\newcommand\xM{\mathscr{M}}
\newcommand\xN{\mathscr{N}}
\newcommand\xO{\mathscr{O}}
\newcommand\xP{\mathscr{P}}
\newcommand\xQ{\mathscr{Q}}
\newcommand\xR{\mathscr{R}}
\newcommand\xS{\mathscr{S}}
\newcommand\xT{\mathscr{T}}
\newcommand\xU{\mathscr{U}}
\newcommand\xV{\mathscr{V}}
\newcommand\xW{\mathscr{W}}
\newcommand\xX{\mathscr{X}}
\newcommand\xY{\mathscr{Y}}
\newcommand\xZ{\mathscr{Z}}

% --------------------
% CALLIGRAPHIC LETTERS
% --------------------
\DeclareMathAlphabet{\mathcal}{OMS}{cmsy}{m}{n}
\newcommand\cA{\mathcal{A}}
\newcommand\cB{\mathcal{B}}
\newcommand\cC{\mathcal{C}}
\newcommand\cD{\mathcal{D}}
\newcommand\cE{\mathcal{E}}
\newcommand\cF{\mathcal{F}}
\newcommand\cG{\mathcal{G}}
\newcommand\cH{\mathcal{H}}
\newcommand\cI{\mathcal{I}}
\newcommand\cJ{\mathcal{J}}
\newcommand\cK{\mathcal{K}}
\newcommand\cL{\mathcal{L}}
\newcommand\cM{\mathcal{M}}
\newcommand\cN{\mathcal{N}}
\newcommand\cO{\mathcal{O}}
\newcommand\cP{\mathcal{P}}
\newcommand\cQ{\mathcal{Q}}
\newcommand\cR{\mathcal{R}}
\newcommand\cS{\mathcal{S}}
\newcommand\cT{\mathcal{T}}
\newcommand\cU{\mathcal{U}}
\newcommand\cV{\mathcal{V}}
\newcommand\cW{\mathcal{W}}
\newcommand\cX{\mathcal{X}}
\newcommand\cY{\mathcal{Y}}
\newcommand\cZ{\mathcal{Z}}

% -------------------------
% BOLD CALLIGRAPHIC LETTERS
% -------------------------
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}
\newcommand\tA{\mathbfcal{A}}
\newcommand\tB{\mathbfcal{B}}
\newcommand\tC{\mathbfcal{C}}
\newcommand\tD{\mathbfcal{D}}
\newcommand\tE{\mathbfcal{E}}
\newcommand\tF{\mathbfcal{F}}
\newcommand\tG{\mathbfcal{G}}
\newcommand\tH{\mathbfcal{H}}
\newcommand\tI{\mathbfcal{I}}
\newcommand\tJ{\mathbfcal{J}}
\newcommand\tK{\mathbfcal{K}}
\newcommand\tL{\mathbfcal{L}}
\newcommand\tM{\mathbfcal{M}}
\newcommand\tN{\mathbfcal{N}}
\newcommand\tO{\mathbfcal{O}}
\newcommand\tP{\mathbfcal{P}}
\newcommand\tQ{\mathbfcal{Q}}
\newcommand\tR{\mathbfcal{R}}
\newcommand\tS{\mathbfcal{S}}
\newcommand\tT{\mathbfcal{T}}
\newcommand\tU{\mathbfcal{U}}
\newcommand\tV{\mathbfcal{V}}
\newcommand\tW{\mathbfcal{W}}
\newcommand\tX{\mathbfcal{X}}
\newcommand\tY{\mathbfcal{Y}}
\newcommand\tZ{\mathbfcal{Z}}



% -----------------
% LETTERS WITH HATS
% -----------------

% use amsxtra package!

\newcommand\Ahat{{\hat A}}
\newcommand\Bhat{{\hat B}}
\newcommand\Chat{{\hat C}}
\newcommand\Dhat{{\hat D}}
\newcommand\Ehat{{\hat E}}
\newcommand\Fhat{{\hat F}}
\newcommand\Ghat{{\hat G}}
\newcommand\Hhat{{\hat H}}
\newcommand\Ihat{{\hat I}}
\newcommand\Jhat{{\hat J}}
\newcommand\Khat{{\hat K}}
\newcommand\Lhat{{\hat L}}
\newcommand\Mhat{{\hat M}}
\newcommand\Nhat{{\hat N}}
\newcommand\Ohat{{\hat O}}
\newcommand\Phat{{\hat P}}
\newcommand\Qhat{{\hat Q}}
\newcommand\Rhat{{\hat R}}
\newcommand\Shat{{\hat S}}
\newcommand\That{{\hat T}}
\newcommand\Uhat{{\hat U}}
\newcommand\Vhat{{\hat V}}
\newcommand\What{{\hat W}}
\newcommand\Xhat{{\hat X}}
\newcommand\Yhat{{\hat Y}}
\newcommand\Zhat{{\hat Z}}

\newcommand\ahat{{\hat a}}
\newcommand\bhat{{\hat b}}
\newcommand\chat{{\hat c}}
\newcommand\dhat{{\hat d}}
\newcommand\ehat{{\hat e}}
\newcommand\fhat{{\hat f}}
\newcommand\ghat{{\hat g}}
\newcommand\hhat{{\hat h}}
\newcommand\ihat{{\hat i}}
\newcommand\jhat{{\hat j}}
\newcommand\khat{{\hat k}}
\newcommand\lhat{{\hat l}}
\newcommand\mhat{{\hat m}}
\newcommand\nhat{{\hat n}}
\newcommand\ohat{{\hat o}}
\newcommand\phat{{\hat p}}
\newcommand\qhat{{\hat q}}
\newcommand\rhat{{\hat r}}
\newcommand\shat{{\hat s}}
\newcommand\that{{\hat t}}
\newcommand\uhat{{\hat u}}
\newcommand\vhat{{\hat v}}
\newcommand\what{{\hat w}}
\newcommand\xhat{{\hat x}}
\newcommand\yhat{{\hat y}}
\newcommand\zhat{{\hat z}}

\newcommand\rhohat{{\hat\rho}}

% -----------------
% LETTERS WITH BARS
% -----------------

\accentedsymbol\Abar{{\bar A}}
\accentedsymbol\Bbar{{\bar B}}
\accentedsymbol\Cbar{{\bar C}}
\accentedsymbol\Dbar{{\bar D}}
\accentedsymbol\Ebar{{\bar E}}
\accentedsymbol\Fbar{{\bar F}}
\accentedsymbol\Gbar{{\bar G}}
\accentedsymbol\Hbar{{\bar H}}
\accentedsymbol\Ibar{{\bar I}}
\accentedsymbol\Jbar{{\bar J}}
\accentedsymbol\Kbar{{\bar K}}
\accentedsymbol\Lbar{{\bar L}}
\accentedsymbol\Mbar{{\bar M}}
\accentedsymbol\Nbar{{\bar N}}
\accentedsymbol\Obar{{\bar O}}
\accentedsymbol\Pbar{{\bar P}}
\accentedsymbol\Qbar{{\bar Q}}
\accentedsymbol\Rbar{{\bar R}}
\accentedsymbol\Sbar{{\bar S}}
\accentedsymbol\Tbar{{\bar T}}
\accentedsymbol\Ubar{{\bar U}}
\accentedsymbol\Vbar{{\bar V}}
\accentedsymbol\Wbar{{\bar W}}
\accentedsymbol\Xbar{{\bar X}}
\accentedsymbol\Ybar{{\bar Y}}
\accentedsymbol\Zbar{{\bar Z}}

\accentedsymbol\abar{{\bar a}}
\accentedsymbol\bbar{{\bar b}}
\accentedsymbol\cbar{{\bar c}}
\accentedsymbol\dbar{{\bar d}}
\accentedsymbol\ebar{{\bar e}}
\accentedsymbol\fbar{{\bar f}}
\accentedsymbol\gbar{{\bar g}}
\makeatletter
\@ifundefined{hbar}{}{
        \let\oldhbar\hbar % we are going to overwrite an existing command; keep the old version
        \let\hbar\@undefined
}
\makeatother
\accentedsymbol\hbar{{\bar h}}
\accentedsymbol\ibar{{\bar i}}
\accentedsymbol\jbar{{\bar j}}
\accentedsymbol\kbar{{\bar k}}
\accentedsymbol\lbar{{\bar l}}
\accentedsymbol\mbar{{\bar m}}
\accentedsymbol\nbar{{\bar n}}
\makeatletter
\@ifundefined{obar}{}{
        \let\oldobar\obar % we are going to overwrite an existing command; keep the old version
        \let\obar\@undefined
}
\makeatother
\accentedsymbol{\obar}{{\bar o}}
\accentedsymbol\pbar{{\bar p}}
\accentedsymbol\qbar{{\bar q}}
\accentedsymbol\rbar{{\bar r}}
\accentedsymbol\sbar{{\bar s}}
\accentedsymbol\tbar{{\bar t}}
\accentedsymbol\ubar{{\bar u}}
\accentedsymbol\vbar{{\bar v}}
\accentedsymbol\wbar{{\bar w}}
\accentedsymbol\xbar{{\bar x}}
\accentedsymbol\ybar{{\bar y}}
\accentedsymbol\zbar{{\bar z}}

% -------------
% GREEK LETTERS
% -------------
\newcommand\eps{\epsilon}


% ---------------------------------
% MATRIX/VECTOR VARIABLES WITH HATS
% ---------------------------------

\accentedsymbol\mAhat{{\hat\mA}}
\accentedsymbol\mBhat{{\hat\mB}}
\accentedsymbol\mChat{{\hat\mC}}
\accentedsymbol\mDhat{{\hat\mD}}
\accentedsymbol\mEhat{{\hat\mE}}
\accentedsymbol\mFhat{{\hat\mF}}
\accentedsymbol\mGhat{{\hat\mG}}
\accentedsymbol\mHhat{{\hat\mH}}
\accentedsymbol\mIhat{{\hat\mI}}
\accentedsymbol\mJhat{{\hat\mJ}}
\accentedsymbol\mKhat{{\hat\mK}}
\accentedsymbol\mLhat{{\hat\mL}}
\accentedsymbol\mMhat{{\hat\mM}}
\accentedsymbol\mNhat{{\hat\mN}}
\accentedsymbol\mOhat{{\hat\mO}}
\accentedsymbol\mPhat{{\hat\mP}}
\accentedsymbol\mQhat{{\hat\mQ}}
\accentedsymbol\mRhat{{\hat\mR}}
\accentedsymbol\mShat{{\hat\mS}}
\accentedsymbol\mThat{{\hat\mT}}
\accentedsymbol\mUhat{{\hat\mU}}
\accentedsymbol\mVhat{{\hat\mV}}
\accentedsymbol\mWhat{{\hat\mW}}
\accentedsymbol\mXhat{{\hat\mX}}
\accentedsymbol\mYhat{{\hat\mY}}
\accentedsymbol\mZhat{{\hat\mZ}}

\accentedsymbol\vahat{{\hat\va}}
\accentedsymbol\vbhat{{\hat\vb}}
\accentedsymbol\vchat{{\hat\vc}}
\accentedsymbol\vdhat{{\hat\vd}}
\accentedsymbol\vehat{{\hat\ve}}
\accentedsymbol\vfhat{{\hat\vf}}
\accentedsymbol\vghat{{\hat\vg}}
\accentedsymbol\vhhat{{\hat\vh}}
\accentedsymbol\vihat{{\hat\vi}}
\accentedsymbol\vjhat{{\hat\vj}}
\accentedsymbol\vkhat{{\hat\vk}}
\accentedsymbol\vlhat{{\hat\vl}}
\accentedsymbol\vmhat{{\hat\vm}}
\accentedsymbol\vnhat{{\hat\vn}}
\accentedsymbol\vohat{{\hat\vo}}
\accentedsymbol\vphat{{\hat\vp}}
\accentedsymbol\vqhat{{\hat\vq}}
\accentedsymbol\vrhat{{\hat\vr}}
\accentedsymbol\vshat{{\hat\vs}}
\accentedsymbol\vthat{{\hat\vt}}
\accentedsymbol\vuhat{{\hat\vu}}
\accentedsymbol\vvhat{{\hat\vv}}
\accentedsymbol\vwhat{{\hat\vw}}
\accentedsymbol\vxhat{{\hat\vx}}
\accentedsymbol\vyhat{{\hat\vy}}
\accentedsymbol\vzhat{{\hat\vz}}

==> emnlp2023/xkeyval.tex <==
%%
%% This is file `xkeyval.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xkeyval.dtx  (with options: `xkvtex')
%% 
%% ---------------------------------------
%% Copyright (C) 2004-2014 Hendri Adriaens
%% ---------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2003/12/01 or later.
%%
%% This work has the LPPL maintenance status "maintained".
%%
%% This Current Maintainer of this work is Hendri Adriaens.
%%
%% This work consists of the file xkeyval.dtx and derived files
%% keyval.tex, xkvtxhdr.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, xkvutils.tex, pst-xkey.tex, pst-xkey.sty, xkveca.cls,
%% xkvecb.cls, xkvesa.sty, xkvesb.sty, xkvesc.sty, xkvex1.tex,
%% xkvex2.tex, xkvex3.tex and xkvex4.tex.
%%
%% The following files constitute the xkeyval bundle and must be
%% distributed as a whole: readme, xkeyval.pdf, keyval.tex,
%% pst-xkey.sty, pst-xkey.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, xkvtxhdr.tex, xkvutils.tex, pst-xkey.dtx and xkeyval.dtx.
%%
\csname XKeyValLoaded\endcsname
\let\XKeyValLoaded\endinput
\edef\XKVcatcodes{%
  \catcode`\noexpand\@\the\catcode`\@\relax
  \catcode`\noexpand\=\the\catcode`\=\relax
  \catcode`\noexpand\,\the\catcode`\,\relax
  \catcode`\noexpand\:\the\catcode`\:\relax
  \let\noexpand\XKVcatcodes\relax
}
\catcode`\@11\relax
\catcode`\=12\relax
\catcode`\,12\relax
\catcode`\:12\relax
\input xkvutils
\newcount\XKV@depth
\newif\ifXKV@st
\newif\ifXKV@sg
\newif\ifXKV@pl
\newif\ifXKV@knf
\newif\ifXKV@rkv
\newif\ifXKV@inpox
\newif\ifXKV@preset
\let\XKV@rm\@empty
\ifx\ProvidesFile\@undefined
  \message{2014/12/03 v2.7a key=value parser (HA)}
  \input xkvtxhdr
\else
  \ProvidesFile{xkeyval.tex}[2014/12/03 v2.7a key=value parser (HA)]
  \@addtofilelist{xkeyval.tex}
\fi
\def\XKV@warn#1{\message{xkeyval warning: #1}}
\def\XKV@err#1{\errmessage{xkeyval error: #1}}
\def\KV@errx{\XKV@err}
\let\KV@err\KV@errx
\def\XKV@ifstar#1{\@ifnextcharacter*{\@firstoftwo{#1}}}
\def\XKV@ifplus#1{\@ifnextcharacter+{\@firstoftwo{#1}}}
\def\XKV@makepf#1{%
  \KV@@sp@def\XKV@prefix{#1}%
  \def\XKV@resa{XKV}%
  \ifx\XKV@prefix\XKV@resa
    \XKV@err{`XKV' prefix is not allowed}%
    \let\XKV@prefix\@empty
  \else
    \edef\XKV@prefix{\ifx\XKV@prefix\@empty\else\XKV@prefix @\fi}%
  \fi
}
\def\XKV@makehd#1{%
  \expandafter\KV@@sp@def\expandafter\XKV@header\expandafter{#1}%
  \edef\XKV@header{%
    \XKV@prefix\ifx\XKV@header\@empty\else\XKV@header @\fi
  }%
}
\def\XKV@srstate#1#2{%
  \ifx\@empty#2\@empty\advance\XKV@depth\@ne\fi
  \XKV@for@n{XKV@prefix,XKV@fams,XKV@tkey,XKV@na,%
    ifXKV@st,ifXKV@pl,ifXKV@knf,CurrentOption}\XKV@resa{%
    \expandafter\let\csname\XKV@resa#1\expandafter
      \endcsname\csname\XKV@resa#2\endcsname
  }%
  \ifx\@empty#1\@empty\advance\XKV@depth\m@ne\fi
}
\def\XKV@testopta#1{%
  \XKV@ifstar{\XKV@sttrue\XKV@t@stopta{#1}}%
    {\XKV@stfalse\XKV@t@stopta{#1}}%
}
\def\XKV@t@stopta#1{\XKV@ifplus{\XKV@pltrue#1}{\XKV@plfalse#1}}
\def\XKV@testoptb#1{\@testopt{\XKV@t@stoptb#1}{KV}}
\def\XKV@t@stoptb#1[#2]#3{%
  \XKV@makepf{#2}%
  \XKV@makehd{#3}%
  \KV@@sp@def\XKV@tfam{#3}%
  #1%
}
\def\XKV@testoptc#1{\@testopt{\XKV@t@stoptc#1}{KV}}
\def\XKV@t@stoptc#1[#2]#3{%
  \XKV@makepf{#2}%
  \XKV@checksanitizeb{#3}\XKV@fams
  \expandafter\XKV@sp@deflist\expandafter
    \XKV@fams\expandafter{\XKV@fams}%
  \@testopt#1{}%
}
\def\XKV@testoptd#1#2{%
  \XKV@testoptb{%
    \edef\XKV@tempa{#2\XKV@header}%
    \def\XKV@tempb{\@testopt{\XKV@t@stoptd#1}}%
    \expandafter\XKV@tempb\expandafter{\XKV@tempa}%
  }%
}
\def\XKV@t@stoptd#1[#2]#3{%
  \@ifnextchar[{\XKV@sttrue#1{#2}{#3}}{\XKV@stfalse#1{#2}{#3}[]}%
}
\def\XKV@ifcmd#1#2#3{%
  \def\XKV@@ifcmd##1#2##2##3\@nil##4{%
    \def##4{##2}\ifx##4\@nnil
      \def##4{##1}\expandafter\@secondoftwo
    \else
      \expandafter\@firstoftwo
    \fi
  }%
  \XKV@@ifcmd#1#2{\@nil}\@nil#3%
}
\def\XKV@getkeyname#1#2{\expandafter\XKV@g@tkeyname#1=\@nil#2}
\long\def\XKV@g@tkeyname#1=#2\@nil#3{%
  \XKV@ifcmd{#1}\savevalue#3{\XKV@rkvtrue\XKV@sgfalse}{%
    \XKV@ifcmd{#1}\gsavevalue#3%
      {\XKV@rkvtrue\XKV@sgtrue}{\XKV@rkvfalse\XKV@sgfalse}%
  }%
}
\def\XKV@getsg#1#2{%
  \expandafter\XKV@ifcmd\expandafter{#1}\global#2\XKV@sgtrue\XKV@sgfalse
}
\def\XKV@define@default#1#2{%
  \expandafter\def\csname\XKV@header#1@default\expandafter
    \endcsname\expandafter{\csname\XKV@header#1\endcsname{#2}}%
}
\def\define@key{\XKV@testoptb\XKV@define@key}
\def\XKV@define@key#1{%
  \@ifnextchar[{\XKV@d@fine@k@y{#1}}{%
    \long\expandafter\def\csname\XKV@header#1\endcsname####1%
  }%
}
\def\XKV@d@fine@k@y#1[#2]{%
  \XKV@define@default{#1}{#2}%
  \expandafter\def\csname\XKV@header#1\endcsname##1%
}
\def\define@cmdkey{\XKV@testoptd\XKV@define@cmdkey{cmd}}
\def\XKV@define@cmdkey#1#2[#3]#4{%
  \ifXKV@st\XKV@define@default{#2}{#3}\fi
  \def\XKV@tempa{\expandafter\def\csname\XKV@header#2\endcsname####1}%
  \begingroup\expandafter\endgroup\expandafter\XKV@tempa\expandafter
    {\expandafter\def\csname#1#2\endcsname{##1}#4}%
}
\def\define@cmdkeys{\XKV@testoptd\XKV@define@cmdkeys{cmd}}
\def\XKV@define@cmdkeys#1#2[#3]{%
  \XKV@sp@deflist\XKV@tempa{#2}%
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \edef\XKV@tempa{\noexpand\XKV@define@cmdkey{#1}{\XKV@tempa}}%
    \XKV@tempa[#3]{}%
  }%
}
\def\define@choicekey{\XKV@testopta{\XKV@testoptb\XKV@define@choicekey}}
\def\XKV@define@choicekey#1{\@testopt{\XKV@d@fine@choicekey{#1}}{}}
\def\XKV@d@fine@choicekey#1[#2]#3{%
  \toks@{#2}%
  \XKV@sp@deflist\XKV@tempa{#3}\XKV@toks\expandafter{\XKV@tempa}%
  \@ifnextchar[{\XKV@d@fine@ch@icekey{#1}}{\XKV@d@fine@ch@ic@key{#1}}%
}
\def\XKV@d@fine@ch@icekey#1[#2]{%
  \XKV@define@default{#1}{#2}%
  \XKV@d@fine@ch@ic@key{#1}%
}
\def\XKV@d@fine@ch@ic@key#1{%
  \ifXKV@pl\XKV@afterelsefi
    \expandafter\XKV@d@f@ne@ch@ic@k@y
  \else\XKV@afterfi
    \expandafter\XKV@d@f@ne@ch@ic@key
  \fi
  \csname\XKV@header#1\endcsname
}
\def\XKV@d@f@ne@ch@ic@key#1#2{\XKV@d@f@n@@ch@ic@k@y#1{{#2}}}
\def\XKV@d@f@ne@ch@ic@k@y#1#2#3{\XKV@d@f@n@@ch@ic@k@y#1{{#2}{#3}}}
\def\XKV@d@f@n@@ch@ic@k@y#1#2{%
  \edef#1##1{%
    \ifXKV@st\noexpand\XKV@sttrue\else\noexpand\XKV@stfalse\fi
    \ifXKV@pl\noexpand\XKV@pltrue\else\noexpand\XKV@plfalse\fi
    \noexpand\XKV@checkchoice[\the\toks@]{##1}{\the\XKV@toks}%
  }%
  \def\XKV@tempa{\def#1####1}%
  \expandafter\XKV@tempa\expandafter{#1{##1}#2}%
}
\def\define@boolkey{\XKV@t@stopta{\XKV@testoptd\XKV@define@boolkey{}}}
\def\XKV@define@boolkey#1#2[#3]{%
  \ifXKV@pl\XKV@afterelsefi
    \expandafter\XKV@d@f@ne@boolkey
  \else\XKV@afterfi
    \expandafter\XKV@d@fine@boolkey
  \fi
  \csname\XKV@header#2\endcsname{#2}{#1#2}{#3}%
}
\def\XKV@d@fine@boolkey#1#2#3#4#5{%
  \XKV@d@f@ne@b@olkey#1{#2}{#3}{#4}%
    {{\csname#3\XKV@resa\endcsname#5}}%
}
\def\XKV@d@f@ne@boolkey#1#2#3#4#5#6{%
  \XKV@d@f@ne@b@olkey#1{#2}{#3}{#4}%
    {{\csname#3\XKV@resa\endcsname#5}{#6}}%
}
\def\XKV@d@f@ne@b@olkey#1#2#3#4#5{%
  \expandafter\newif\csname if#3\endcsname
  \ifXKV@st\XKV@define@default{#2}{#4}\fi
  \ifXKV@pl
    \def#1##1{\XKV@pltrue\XKV@sttrue
      \XKV@checkchoice[\XKV@resa]{##1}{true,false}#5%
    }%
  \else
    \def#1##1{\XKV@plfalse\XKV@sttrue
      \XKV@checkchoice[\XKV@resa]{##1}{true,false}#5%
    }%
  \fi
}
\def\define@boolkeys{\XKV@plfalse\XKV@testoptd\XKV@define@boolkeys{}}
\def\XKV@define@boolkeys#1#2[#3]{%
  \XKV@sp@deflist\XKV@tempa{#2}%
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \expandafter\XKV@d@fine@boolkeys\expandafter{\XKV@tempa}{#1}{#3}%
  }%
}
\def\XKV@d@fine@boolkeys#1#2#3{%
  \expandafter\XKV@d@f@ne@b@olkey\csname\XKV@header#1\endcsname
    {#1}{#2#1}{#3}{{\csname#2#1\XKV@resa\endcsname}}%
}
\def\XKV@cc{\XKV@testopta{\@testopt\XKV@checkchoice{}}}
\def\XKV@checkchoice[#1]#2#3{%
  \def\XKV@tempa{#1}%
  \ifXKV@st\lowercase{\fi
  \ifx\XKV@tempa\@empty
    \def\XKV@tempa{\XKV@ch@ckch@ice\@nil{#2}{#3}}%
  \else
    \def\XKV@tempa{\XKV@ch@ckchoice#1\@nil{#2}{#3}}%
  \fi
  \ifXKV@st}\fi\XKV@tempa
}
\def\XKV@ch@ckchoice#1#2\@nil#3#4{%
  \def\XKV@tempa{#2}%
  \ifx\XKV@tempa\@empty\XKV@afterelsefi
    \XKV@ch@ckch@ice#1{#3}{#4}%
  \else\XKV@afterfi
    \XKV@@ch@ckchoice#1#2{#3}{#4}%
  \fi
}
\def\XKV@ch@ckch@ice#1#2#3{%
  \def\XKV@tempa{#1}%
  \ifx\XKV@tempa\@nnil\let\XKV@tempa\@empty\else
    \def\XKV@tempa{\def#1{#2}}%
  \fi
  \in@{,#2,}{,#3,}%
  \ifin@
    \ifXKV@pl
      \XKV@addtomacro@n\XKV@tempa\@firstoftwo
    \else
      \XKV@addtomacro@n\XKV@tempa\@firstofone
    \fi
  \else
    \ifXKV@pl
      \XKV@addtomacro@n\XKV@tempa\@secondoftwo
    \else
      \XKV@toks{#2}%
      \XKV@err{value `\the\XKV@toks' is not allowed}%
      \XKV@addtomacro@n\XKV@tempa\@gobble
    \fi
  \fi
  \XKV@tempa
}
\def\XKV@@ch@ckchoice#1#2#3#4{%
  \edef\XKV@tempa{\the\count@}\count@\z@
  \def\XKV@tempb{#3}%
  \def\XKV@tempc##1,{%
    \def#1{##1}%
    \ifx#1\@nnil
      \def#1{#3}\def#2{-1}\count@\XKV@tempa
      \ifXKV@pl
        \let\XKV@tempd\@secondoftwo
      \else
        \XKV@toks{#3}%
        \XKV@err{value `\the\XKV@toks' is not allowed}%
        \let\XKV@tempd\@gobble
      \fi
    \else
      \ifx#1\XKV@tempb
        \edef#2{\the\count@}\count@\XKV@tempa
        \ifXKV@pl
          \let\XKV@tempd\XKV@@ch@ckch@ice
        \else
          \let\XKV@tempd\XKV@@ch@ckch@ic@
        \fi
      \else
        \advance\count@\@ne
        \let\XKV@tempd\XKV@tempc
      \fi
    \fi
    \XKV@tempd
  }%
  \XKV@tempc#4,\@nil,%
}
\def\XKV@@ch@ckch@ice#1\@nil,{\@firstoftwo}
\def\XKV@@ch@ckch@ic@#1\@nil,{\@firstofone}
\def\key@ifundefined{\@testopt\XKV@key@ifundefined{KV}}
\def\XKV@key@ifundefined[#1]#2{%
  \XKV@makepf{#1}%
  \XKV@checksanitizeb{#2}\XKV@fams
  \expandafter\XKV@sp@deflist\expandafter
    \XKV@fams\expandafter{\XKV@fams}%
  \XKV@key@if@ndefined
}
\def\XKV@key@if@ndefined#1{%
  \XKV@knftrue
  \KV@@sp@def\XKV@tkey{#1}%
  \XKV@whilist\XKV@fams\XKV@tfam\ifXKV@knf\fi{%
    \XKV@makehd\XKV@tfam
    \XKV@ifundefined{\XKV@header\XKV@tkey}{}{\XKV@knffalse}%
  }%
  \ifXKV@knf
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
}
\def\disable@keys{\XKV@testoptb\XKV@disable@keys}
\def\XKV@disable@keys#1{%
  \XKV@checksanitizeb{#1}\XKV@tempa
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \XKV@ifundefined{\XKV@header\XKV@tempa}{%
      \XKV@err{key `\XKV@tempa' undefined}%
    }{%
      \edef\XKV@tempb{%
        \noexpand\XKV@warn{key `\XKV@tempa' has been disabled}%
      }%
      \XKV@ifundefined{\XKV@header\XKV@tempa @default}{%
        \edef\XKV@tempc{\noexpand\XKV@define@key{\XKV@tempa}}%
      }{%
        \edef\XKV@tempc{\noexpand\XKV@define@key{\XKV@tempa}[]}%
      }%
      \expandafter\XKV@tempc\expandafter{\XKV@tempb}%
    }%
  }%
}
\def\presetkeys{\XKV@stfalse\XKV@testoptb\XKV@presetkeys}
\def\gpresetkeys{\XKV@sttrue\XKV@testoptb\XKV@presetkeys}
\def\XKV@presetkeys#1#2{%
  \XKV@pr@setkeys{#1}{preseth}%
  \XKV@pr@setkeys{#2}{presett}%
}
\def\XKV@pr@setkeys#1#2{%
  \XKV@ifundefined{XKV@\XKV@header#2}{%
    \XKV@checksanitizea{#1}\XKV@tempa
    \ifXKV@st\expandafter\global\fi\expandafter\def\csname
      XKV@\XKV@header#2\expandafter\endcsname\expandafter{\XKV@tempa}%
  }{%
    \expandafter\XKV@merge\csname XKV@\XKV@header
      #2\endcsname{#1}\XKV@getkeyname
  }%
}
\def\delpresetkeys{\XKV@stfalse\XKV@testoptb\XKV@delpresetkeys}
\def\gdelpresetkeys{\XKV@sttrue\XKV@testoptb\XKV@delpresetkeys}
\def\XKV@delpresetkeys#1#2{%
  \XKV@d@lpresetkeys{#1}{preseth}%
  \XKV@d@lpresetkeys{#2}{presett}%
}
\def\XKV@d@lpresetkeys#1#2{%
  \XKV@ifundefined{XKV@\XKV@header#2}{%
    \XKV@err{no presets defined for `\XKV@header'}%
  }{%
    \expandafter\XKV@delete\csname XKV@\XKV@header
      #2\endcsname{#1}\XKV@getkeyname
  }%
}
\def\unpresetkeys{\XKV@stfalse\XKV@testoptb\XKV@unpresetkeys}
\def\gunpresetkeys{\XKV@sttrue\XKV@testoptb\XKV@unpresetkeys}
\def\XKV@unpresetkeys{%
  \XKV@ifundefined{XKV@\XKV@header preseth}{%
    \XKV@err{no presets defined for `\XKV@header'}%
  }{%
    \ifXKV@st\expandafter\global\fi\expandafter\let
      \csname XKV@\XKV@header preseth\endcsname\@undefined
    \ifXKV@st\expandafter\global\fi\expandafter\let
      \csname XKV@\XKV@header presett\endcsname\@undefined
  }%
}
\def\savekeys{\XKV@stfalse\XKV@testoptb\XKV@savekeys}
\def\gsavekeys{\XKV@sttrue\XKV@testoptb\XKV@savekeys}
\def\XKV@savekeys#1{%
  \XKV@ifundefined{XKV@\XKV@header save}{%
    \XKV@checksanitizeb{#1}\XKV@tempa
    \ifXKV@st\expandafter\global\fi\expandafter\def\csname XKV@%
      \XKV@header save\expandafter\endcsname\expandafter{\XKV@tempa}%
  }{%
    \expandafter\XKV@merge\csname XKV@\XKV@header
      save\endcsname{#1}\XKV@getsg
  }%
}
\def\delsavekeys{\XKV@stfalse\XKV@testoptb\XKV@delsavekeys}
\def\gdelsavekeys{\XKV@sttrue\XKV@testoptb\XKV@delsavekeys}
\def\XKV@delsavekeys#1{%
  \XKV@ifundefined{XKV@\XKV@header save}{%
    \XKV@err{no save keys defined for `\XKV@header'}%
  }{%
    \expandafter\XKV@delete\csname XKV@\XKV@header
      save\endcsname{#1}\XKV@getsg
  }%
}
\def\unsavekeys{\XKV@stfalse\XKV@testoptb\XKV@unsavekeys}
\def\gunsavekeys{\XKV@sttrue\XKV@testoptb\XKV@unsavekeys}
\def\XKV@unsavekeys{%
  \XKV@ifundefined{XKV@\XKV@header save}{%
    \XKV@err{no save keys defined for `\XKV@header'}%
  }{%
    \ifXKV@st\expandafter\global\fi\expandafter\let
      \csname XKV@\XKV@header save\endcsname\@undefined
  }%
}
\def\setkeys{\XKV@testopta{\XKV@testoptc\XKV@setkeys}}
\long\def\XKV@setkeys[#1]#2{%
  \XKV@checksanitizea{#2}\XKV@resb
  \let\XKV@naa\@empty
  \XKV@for@o\XKV@resb\XKV@tempa{%
    \expandafter\XKV@g@tkeyname\XKV@tempa=\@nil\XKV@tempa
    \XKV@addtolist@x\XKV@naa\XKV@tempa
  }%
  \ifnum\XKV@depth=\z@\let\XKV@rm\@empty\fi
  \XKV@usepresetkeys{#1}{preseth}%
  \expandafter\XKV@s@tkeys\expandafter{\XKV@resb}{#1}%
  \XKV@usepresetkeys{#1}{presett}%
  \let\CurrentOption\@empty
}
\def\XKV@usepresetkeys#1#2{%
  \XKV@presettrue
  \XKV@for@eo\XKV@fams\XKV@tfam{%
    \XKV@makehd\XKV@tfam
    \XKV@ifundefined{XKV@\XKV@header#2}{}{%
      \XKV@toks\expandafter\expandafter\expandafter
        {\csname XKV@\XKV@header#2\endcsname}%
      \@expandtwoargs\XKV@s@tkeys{\the\XKV@toks}%
        {\XKV@naa\ifx\XKV@naa\@empty\else,\fi#1}%
    }%
  }%
  \XKV@presetfalse
}
\long\def\XKV@s@tkeys#1#2{%
  \XKV@sp@deflist\XKV@na{#2}%
  \XKV@for@n{#1}\CurrentOption{%
    \expandafter\XKV@s@tk@ys\CurrentOption==\@nil
  }%
}
\long\def\XKV@s@tk@ys#1=#2=#3\@nil{%
  \XKV@g@tkeyname#1=\@nil\XKV@tkey
  \expandafter\KV@@sp@def\expandafter\XKV@tkey\expandafter{\XKV@tkey}%
  \ifx\XKV@tkey\@empty
    \XKV@toks{#2}%
    \ifcat$\the\XKV@toks$\else
      \XKV@err{no key specified for value `\the\XKV@toks'}%
    \fi
  \else
    \@expandtwoargs\in@{,\XKV@tkey,}{,\XKV@na,}%
    \ifin@\else
      \XKV@knftrue
      \KV@@sp@def\XKV@tempa{#2}%
      \ifXKV@preset\XKV@s@tk@ys@{#3}\else
        \ifXKV@pl
          \XKV@for@eo\XKV@fams\XKV@tfam{%
            \XKV@makehd\XKV@tfam
            \XKV@s@tk@ys@{#3}%
          }%
        \else
          \XKV@whilist\XKV@fams\XKV@tfam\ifXKV@knf\fi{%
            \XKV@makehd\XKV@tfam
            \XKV@s@tk@ys@{#3}%
          }%
        \fi
      \fi
      \ifXKV@knf
        \ifXKV@inpox
          \ifx\XKV@doxs\relax
            \ifx\@currext\@clsextension\else
              \let\CurrentOption\XKV@tkey\@unknownoptionerror
            \fi
          \else\XKV@doxs\fi
        \else
          \ifXKV@st
            \XKV@addtolist@o\XKV@rm\CurrentOption
          \else
            \XKV@err{`\XKV@tkey' undefined in families `\XKV@fams'}%
          \fi
        \fi
      \else
        \ifXKV@inpox\ifx\XKV@testclass\XKV@documentclass
          \expandafter\XKV@useoption\expandafter{\CurrentOption}%
        \fi\fi
      \fi
    \fi
  \fi
}
\def\XKV@s@tk@ys@#1{%
  \XKV@ifundefined{\XKV@header\XKV@tkey}{}{%
    \XKV@knffalse
    \XKV@ifundefined{XKV@\XKV@header save}{}{%
      \expandafter\XKV@testsavekey\csname XKV@\XKV@header
        save\endcsname\XKV@tkey
    }%
    \ifXKV@rkv
      \ifXKV@sg\expandafter\global\fi\expandafter\let
        \csname XKV@\XKV@header\XKV@tkey @value\endcsname\XKV@tempa
    \fi
    \expandafter\XKV@replacepointers\expandafter{\XKV@tempa}%
    \ifx\@empty#1\@empty\XKV@afterelsefi
      \XKV@ifundefined{\XKV@header\XKV@tkey @default}{%
        \XKV@err{no value specified for key `\XKV@tkey'}%
      }{%
        \expandafter\expandafter\expandafter\XKV@default
          \csname\XKV@header\XKV@tkey @default\endcsname\@nil
      }%
    \else\XKV@afterfi
      \XKV@srstate{@\romannumeral\XKV@depth}{}%
      \csname\XKV@header\XKV@tkey\expandafter
        \endcsname\expandafter{\XKV@tempa}\relax
      \XKV@srstate{}{@\romannumeral\XKV@depth}%
    \fi
  }%
}
\def\XKV@testsavekey#1#2{%
  \ifXKV@rkv\else
    \XKV@for@o#1\XKV@resa{%
      \expandafter\XKV@ifcmd\expandafter{\XKV@resa}\global\XKV@resa{%
        \ifx#2\XKV@resa
          \XKV@rkvtrue\XKV@sgtrue
        \fi
      }{%
        \ifx#2\XKV@resa
          \XKV@rkvtrue\XKV@sgfalse
        \fi
      }%
    }%
  \fi
}
\long\def\XKV@replacepointers#1{%
  \let\XKV@tempa\@empty
  \let\XKV@resa\@empty
  \XKV@r@placepointers#1\usevalue\@nil
}
\long\def\XKV@r@placepointers#1\usevalue#2{%
  \XKV@addtomacro@n\XKV@tempa{#1}%
  \def\XKV@tempb{#2}%
  \ifx\XKV@tempb\@nnil\else\XKV@afterfi
    \XKV@ifundefined{XKV@\XKV@header#2@value}{%
      \XKV@err{no value recorded for key `#2'; ignored}%
      \XKV@r@placepointers
    }{%
      \@expandtwoargs\in@{,#2,}{,\XKV@resa,}%
      \ifin@\XKV@afterelsefi
        \XKV@err{back linking pointers; pointer replacement canceled}%
      \else\XKV@afterfi
        \XKV@addtolist@x\XKV@resa{#2}%
        \expandafter\expandafter\expandafter\XKV@r@placepointers
          \csname XKV@\XKV@header#2@value\endcsname
      \fi
    }%
  \fi
}
\def\XKV@default#1#2\@nil{%
  \expandafter\edef\expandafter\XKV@tempa
    \expandafter{\expandafter\@gobble\string#1}%
  \edef\XKV@tempb{\XKV@header\XKV@tkey}%
  \@onelevel@sanitize\XKV@tempb
  \ifx\XKV@tempa\XKV@tempb
    \begingroup
      \expandafter\def\csname\XKV@header\XKV@tkey\endcsname##1{%
        \gdef\XKV@tempa{##1}%
      }%
      \csname\XKV@header\XKV@tkey @default\endcsname
    \endgroup
    \XKV@ifundefined{XKV@\XKV@header save}{}{%
      \expandafter\XKV@testsavekey\csname XKV@\XKV@header
        save\endcsname\XKV@tkey
    }%
    \ifXKV@rkv
      \ifXKV@sg\expandafter\global\fi\expandafter\let
        \csname XKV@\XKV@header\XKV@tkey @value\endcsname\XKV@tempa
    \fi
    \expandafter\XKV@replacepointers\expandafter
      {\XKV@tempa}\XKV@afterelsefi
    \XKV@srstate{@\romannumeral\XKV@depth}{}%
    \expandafter#1\expandafter{\XKV@tempa}\relax
    \XKV@srstate{}{@\romannumeral\XKV@depth}%
  \else\XKV@afterfi
    \XKV@srstate{@\romannumeral\XKV@depth}{}%
    \csname\XKV@header\XKV@tkey @default\endcsname\relax
    \XKV@srstate{}{@\romannumeral\XKV@depth}%
  \fi
}
\def\setrmkeys{\XKV@testopta{\XKV@testoptc\XKV@setrmkeys}}
\def\XKV@setrmkeys[#1]{%
  \def\XKV@tempa{\XKV@setkeys[#1]}%
  \expandafter\XKV@tempa\expandafter{\XKV@rm}%
}
\XKVcatcodes
\endinput
%%
%% End of file `xkeyval.tex'.


==> main/small-macros.tex <==
% File: macros.tex
%
% Contains general macros for use with LaTeX.
%
% $LastChangedRevision: 961 $
% $LastChangedDate: 2008-08-25 18:43:18 +0200 (Mon, 25 Aug 2008) $
%
% Author: Rainer Gemulla
%
% Packages:
% \usepackage{array}
% \usepackage{amsxtra}



% this is just the default macros file with some commented out



% --------------
% EDITING MACROS
% --------------
%\newcommand{\todo}[1]{\textcolor{red}{#1}} % todos
\newcommand{\co}[1]{\textcolor{blue}{#1}} % comments
\newcommand{\eat}[1]{} % TO MAKE LARGE BLOCKS OF TEXT INVISIBLE

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\dgreen}[1]{\textcolor{green!70!black}{#1}}
\newcommand{\orange}[1]{\textcolor{orange}{#1}}
\newcommand{\yellow}[1]{\textcolor[rgb]{102, 77, 0}{#1}}

% -------------
% CARDINALITIES
% -------------
\newcommand{\sz}[1]{\lvert#1\rvert}   % cardinality of set
\newcommand{\card}[1]{\lvert#1\rvert} % cardinality of set
\newcommand{\Sz}[1]{\lVert#1\rVert}   % cardinality of set, distinct (not used in thesis!)
\newcommand{\Card}[1]{\lVert#1\rVert} % cardinality of set, distinct (not used in thesis!)

% ----------
% EQUALITIES
% ----------
\newcommand{\eqdef}{\stackrel{\mathrm{def}}{=}} % definining equality
\newcommand{\eqdot}{\doteq} % APPROACHES THE LIMIT (asymptotic equality)
\newcommand{\eqdist}{\equiv} % equality in distribution

% --------
% ROUNDING
% --------
\newcommand{\floor}[1]{\left\lfloor#1\right\rfloor} % floor, automatic brackets
\newcommand{\floorn}[1]{\lfloor#1\rfloor} % floor, normal brackets
\newcommand{\ceil}[1]{\left\lceil#1\right\rceil} % ceil, automatic brackets
\newcommand{\ceiln}[1]{\lceil#1\rceil} % ceil, normal brackets

% ---------------
% ABSOLUTE VALUES
% ---------------
\newcommand{\abs}[1]{\left\lvert#1\right\rvert} % abs, automatic brackets
\newcommand{\absn}[1]{\lvert#1\rvert} % abs, normal brackets

% ---------------------
% SUPER- AND SUBSCRIPTS
% ---------------------
\newcommand{\td}[2]{\if*#1\else^{#1}\fi\if*#2\else_{#2}\fi} % ^?_?, *=ignore

% -----------
% PROBABILITY
% -----------
\newcommand{\xpr}[2]{p\td{#1}{#2}} % Pr^?_?
\newcommand{\uxpr}[2]{\tilde p\td{#1}{#2}} % ~Pr^?_?
\newcommand{\pr}[1]{\xpr**\!\left(#1\right)} % Pr(?], automatic brackets
\newcommand{\prn}[1]{\xpr**\!(#1)} % Pr(?], normal brackets
\newcommand{\prbig}[1]{\xpr**\!\bigl(#1\bigr)} % Pr(?], big brackets
\newcommand{\prBig}[1]{\xpr**\!\Bigl(#1\Bigr)} % Pr(?], Big brackets
\newcommand{\prbigg}[1]{\xpr**\!\biggl(#1\biggr)} % Pr(?], bigg brackets
\newcommand{\prBigg}[1]{\xpr**\!\Biggl(#1\Biggr)} % Pr(?], Bigg brackets

\newcommand{\prf}[3]{\xpr{#1}{#2}\!\left(#3\right)} % Pr^?_?(?), automatic brackets
\newcommand{\uprf}[3]{\uxpr{#1}{#2}\!\left(#3\right)} % ~Pr^?_?(?), automatic brackets

\newcommand{\prs}[1]{\xpr**\!\left(#1\right)} % Pr(?], automatic brackets, no spacing
\newcommand{\prsn}[1]{\xpr**\!(#1)} % Pr(?], normal brackets, no spacing

\newcommand{\Pa}{\operatorname{Pa}}
\newcommand{\Nd}{\operatorname{NonDescendants}}

% -------------
% SPACING
% -------------
\newcommand\macrospace{}

% --------------
% EXPECTED VALUE
% --------------
\newcommand{\xev}[2]{\operatorname{E}\td{#1}{#2}} % E^?_?

\newcommand{\evf}[3]{\xev{#1}{#2}{\left[\macrospace{}#3\macrospace{}\right]}} % E^?_?[?], automatic brackets
\newcommand{\evfn}[3]{\xev{#1}{#2}{[\macrospace{}#3\macrospace{}]}} % E^?_?[?], normal brackets
\newcommand{\evfbig}[3]{\xev{#1}{#2}{\bigl[\macrospace{}#3\macrospace{}\bigr]}} % E^?_?[?], big brackets
\newcommand{\evfBig}[3]{\xev{#1}{#2}{\Bigl[\macrospace{}#3\macrospace{}\Bigr]}} % E^?_?[?], Big brackets
\newcommand{\evfbigg}[3]{\xev{#1}{#2}{\biggl[\macrospace{}#3\macrospace{}\biggr]}} % E^?_?[?], bigg brackets

\newcommand{\ev}[1]{\evf**{#1}} % E[?], automatic brackets
\newcommand{\evn}[1]{\evfn**{#1}} % E[?], normal brackets
\newcommand{\evbig}[1]{\evfbig**{#1}} % E[?], big brackets
\newcommand{\evBig}[1]{\evfBig**{#1}} % E[?], Big brackets
\newcommand{\evbigg}[1]{\evfbigg**{#1}} % E[?], bigg brackets

% ----
% BIAS
% ----
\newcommand{\xbias}[2]{\operatorname{bias}\td{#1}{#2}} % Bias^?_?
\newcommand{\bias}[1]{\xbias**\left[\macrospace{}#1\macrospace{}\right]} % Bias[?], automatic brackets
\newcommand{\biasn}[1]{\xbias**[\macrospace{}#1\macrospace{}]} % Bias[?], normal brackets

% --------
% VARIANCE
% --------
\newcommand{\xvar}[2]{\operatorname{var}\td{#1}{#2}} % Var^?_?
\newcommand{\var}[1]{\xvar**\left[\macrospace{}#1\macrospace{}\right]} % Var[?], automatic brackets
\newcommand{\varn}[1]{\xvar**[\macrospace{}#1\macrospace{}]} % Var[?], normal brackets
\newcommand{\varbig}[1]{\xvar**\bigl[\macrospace{}#1\macrospace{}\bigr]} % Var[?], big brackets
\newcommand{\varBig}[1]{\xvar**\Bigl[\macrospace{}#1\macrospace{}\Bigr]} % Var[?], Big brackets

\newcommand{\xhatvar}[2]{\operatorname{\hat{v}ar}\td{#1}{#2}} % ~Var^?_?
\newcommand{\hatvar}[1]{\xhatvar**\left[\macrospace{}#1\macrospace{}\right]} % ~Var[?], automatic brackets
\newcommand{\hatvarn}[1]{\xhatvar**[\macrospace{}#1\macrospace{}]} % ~Var[?], normal brackets
\newcommand{\hatvarBig}[1]{\xhatvar**\Bigl[\macrospace{}#1\macrospace{}\Bigr]} % ~Var[?], Big brackets

\newcommand{\varf}[3]{\xvar{#1}{#2}{\left[\macrospace{}#3\macrospace{}\right]}} % Var^?_?[?], automatic brackets
\newcommand{\varfn}[3]{\xvar{#1}{#2}{[\macrospace{}#3\macrospace{}]}} % E^?_?[?], normal brackets
\newcommand{\varfbig}[3]{\xvar{#1}{#2}{\bigl[\macrospace{}#3\macrospace{}\bigr]}} % E^?_?[?], big brackets
\newcommand{\varfBig}[3]{\xvar{#1}{#2}{\Bigl[\macrospace{}#3\macrospace{}\Bigr]}} % E^?_?[?], Big brackets
\newcommand{\varfbigg}[3]{\xvar{#1}{#2}{\biggl[\macrospace{}#3\macrospace{}\biggr]}} % E^?_?[?], bigg

% ----------
% COVARIANCE
% ----------
\newcommand{\xcov}[2]{\operatorname{Cov}\td{#1}{#2}} % Cov^?_?
\newcommand{\cov}[1]{\xcov**\left[\macrospace{}#1\macrospace{}\right]} % Cov[?], automatic brackets
\newcommand{\covn}[1]{\xcov**[\macrospace{}#1\macrospace{}]} % Cov[?], normal brackets
\newcommand{\covBig}[1]{\xcov**\Bigl[\macrospace{}#1\macrospace{}\Bigr]} % Cov[?], Big brackets

\newcommand{\xhatcov}[2]{\operatorname{\hat{C}ov}\td{#1}{#2}} % ~Cov^?_?
\newcommand{\hatcov}[1]{\xhatcov**\left[\macrospace{}#1\macrospace{}\right]} % ~Cov[?], automatic brackets
\newcommand{\hatcovn}[1]{\xhatcov**[\macrospace{}#1\macrospace{}]} % ~Cov[?], normal brackets
\newcommand{\hatcovBig}[1]{\xhatcov**\Bigl[\macrospace{}#1\macrospace{}\Bigr]} % ~Cov[?], Big brackets

% --------------
% STANDARD ERROR
% --------------

\newcommand{\xse}[2]{\operatorname{SE}\td{#1}{#2}} % SE^?_?
\newcommand{\se}[1]{\xse**\left[\macrospace{}#1\macrospace{}\right]} % SE[?], automatic brackets
\newcommand{\sen}[1]{\xse**[\macrospace{}#1\macrospace{}]} % SE[?], normal brackets

\newcommand{\xhatse}[2]{\operatorname{\hat{S}E}\td{#1}{#2}} % ~SE^?_?
\newcommand{\hatse}[1]{\xhatse**\left[\macrospace{}#1\macrospace{}\right]} % ~SE[?], automatic brackets
\newcommand{\hatsen}[1]{\xhatse**[\macrospace{}#1\macrospace{}]} % ~SE[?], normal brackets

% --------------
% STANDARD ERROR
% --------------

\newcommand{\xsd}[2]{\operatorname{SD}\td{#1}{#2}} % SD^?_?
\newcommand{\sd}[1]{\xsd**\left[\macrospace{}#1\macrospace{}\right]} % SD[?], automatic brackets
\newcommand{\sdn}[1]{\xsd**[\macrospace{}#1\macrospace{}]} % SD[?], normal brackets

\newcommand{\xhatsd}[2]{\operatorname{\hat{S}D}\td{#1}{#2}} % ~SD^?_?
\newcommand{\hatsd}[1]{\xhatsd**\left[\macrospace{}#1\macrospace{}\right]} % ~SD[?], automatic brackets
\newcommand{\hatsed}[1]{\xhatsd**[\macrospace{}#1\macrospace{}]} % ~SD[?], normal brackets


% ------------------------
% COEFFICIENT OF VARIATION
% ------------------------
\newcommand{\xcv}[2]{\operatorname{CV}\td{#1}{#2}} % Cv^?_?
\newcommand{\cv}[1]{\xcv**\left[\macrospace{}#1\macrospace{}\right]} % Cv[?], automatic brackets
\newcommand{\cvn}[1]{\xcv**[\macrospace{}#1\macrospace{}]} % Var[?], normal brackets
\newcommand{\cvbig}[1]{\xcv**\bigl[\macrospace{}#1\macrospace{}\bigr]} % Cv[?], big brackets
\newcommand{\cvBig}[1]{\xcv**\Bigl[\macrospace{}#1\macrospace{}\Bigr]} % Cv[?], Big brackets

% -----------------
% MEAN SQUARE ERROR
% -----------------
\newcommand{\xmse}[2]{\operatorname{mse}\td{#1}{#2}} % MSE^?_?
\newcommand{\mse}[1]{\xmse**\left[\macrospace{}#1\macrospace{}\right]} % MSE[?], automatic brackets
\newcommand{\msen}[1]{\xmse**[\macrospace{}#1\macrospace{}]} % MSE[?], normal brackets

% ----------------------
% ROOT MEAN SQUARE ERROR
% ----------------------
\newcommand{\xrmse}[2]{\operatorname{rmse}\td{#1}{#2}} % RMSE^?_?
\newcommand{\rmse}[1]{\xrmse**\left[\macrospace{}#1\macrospace{}\right]} % RMSE[?], automatic brackets
\newcommand{\rmsen}[1]{\xrmse**[\macrospace{}#1\macrospace{}]} % RMSE[?], normal brackets

% ----------------------
% AVERAGE RELATIVE ERROR
% ----------------------
\newcommand{\xare}[2]{\operatorname{ARE}\td{#1}{#2}} % ARE^?_?
\newcommand{\are}[1]{\xare**\left[\macrospace{}#1\macrospace{}\right]} % ARE[?], automatic brackets
\newcommand{\aren}[1]{\xare**[\macrospace{}#1\macrospace{}]} % ARE[?], normal brackets

% ---------------------
% BINOMIAL DISTRIBUTION
% ---------------------

% B(k; N,q)
\newcommand{\pbinom}[3]{B\!\left(#1;\,#2,#3\right)} % binomial probability, automatic brackets

% ---------------------------
% HYPERGEOMETRIC DISTRIBUTION
% ---------------------------
\newcommand{\phyper}[4]{H\!\left(#1;\,#2,#3,#4\right)} % hypergeometric probability, automatic brackets

% --------------
% ARGMIN, ARGMAX
% --------------
%\DeclareMathOperator*{\argmin}{argmin} % amsmath package required
%\DeclareMathOperator*{\argmax}{argmax} % amsmath package required

% ----
% SETS
% ----
\renewcommand\:{\colon} % for use with \sset, etc.
\newcommand{\sset}[1]{\left\{\,#1\,\right\}} % { ? }, automatic brackets
\newcommand{\ssets}[1]{\left\{#1\right\}} % {?}, automatic brackets
\newcommand{\ssetn}[1]{\{\,#1\,\}} % { ? }, normal brackets

\newcommand{\comp}[1]{\bar{#1}} % complement

\newcommand{\powerset}[1]{\cP\!\left(#1\right)} % powerset, automatic brackets

\newcommand\adots{{\ensuremath ..}} % short array notation as in A[i..j]

\newcommand{\Nat}{{\ensuremath \bN}}
\newcommand{\Bool}{{\ensuremath \{0,1\}}}

% --------
% BOOLEANS
% --------
\newcommand\true{\text{true}} % use in math mode
\newcommand\false{\text{false}} % use in math mode

% --------------------
% RELATIONAL OPERATORS
% --------------------
\newcommand\join\Join % normal join

% uses txfonts for left/right semi join symbols (and nothing else)
\DeclareSymbolFont{txsymbolsC}{U}{txsyc}{m}{n}
\SetSymbolFont{txsymbolsC}{bold}{U}{txsyc}{bx}{n}
\DeclareFontSubstitution{U}{txsyc}{m}{n}
\DeclareMathSymbol{\ljoin}{\mathrel}{txsymbolsC}{88}
\DeclareMathSymbol{\rjoin}{\mathrel}{txsymbolsC}{89}
%\DeclareMathSymbol{\join}{\mathrel}{txsymbolsC}{90} NOT NEEDED

% -----------
% SQL queries
% -----------
\newcommand{\sql}[1]{\texttt{#1}}

% -------------------
% MULTISET OPERATIONS
% -------------------
\newcommand\mcup{\uplus}       % multiset union
\newcommand\bigmcup{\biguplus} % multiset union, big
\newcommand\mcap{\nplus}       % multiset intersection
\newcommand\bigmcap{\nbigplus} % multiset intersection, big

\newsavebox\setminusbox
\newlength\setminuslen
\newcommand\msetminus{{\savebox{\setminusbox}{$\setminus$}\settowidth{\setminuslen}{\usebox{\setminusbox}}\,\usebox{\setminusbox}\hspace{-.5\setminuslen}^+}} % multiset difference
\newcommand\msetminusl{{\savebox{\setminusbox}{$_\setminus$}\settowidth{\setminuslen}{\usebox{\setminusbox}}\setminus\hspace{-.5\setminuslen}^+}} % multiset difference, when used as subscript


% -----------------
% MATRIX OPERATIONS
% -----------------
\newcommand\xdiag{\operatorname{diag}}
\newcommand\diag[1]{\xdiag\left(#1\right)}    % diagonal matrix
\newcommand\diagn[1]{\xdiag(#1)}    % diagonal matrix, normal brackets
\newcommand\xrank{\operatorname{rank}}
\newcommand\rank[1]{\xrank\left(#1\right)}
\newcommand\rankn[1]{\xrank(#1)}

% determinant: \det

\newcommand\T{\top}
\newcommand\transpose[1]{#1^{\T}}
\newcommand\tr[1]{#1^{\textrm{T}}}
%\newcommand\norm[1]{\left\lVert #1 \right\rVert}
\newcommand\normn[1]{\lVert #1 \rVert}
\newcommand\fnorm[1]{\left\lVert #1 \right\rVert_\text{F}}
\newcommand\fnormn[1]{\lVert #1 \rVert_\text{F}}
\newcommand\rsim{\stackrel{\mathrm{row}}{\sim}}
\newcommand\csim{\stackrel{\mathrm{col}}{\sim}}


% --------------------------
% TABULAR COLUMNS, MATH MODE
% --------------------------

\newcolumntype{C}{>{$\displaystyle}c<{$}} % centered math
\newcolumntype{L}{>{$\displaystyle}l<{$}} % left math
\newcolumntype{R}{>{$\displaystyle}r<{$}} % right math
\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}} % hide column

% extra spacing for math tables (used for after math rows set in display style if no rule follows)
\newcommand{\mathls}{\addlinespace[5pt]}

\newcommand{\mlsideways}[1]{\begin{sideways}\centering\begin{tabular}{c}#1\end{tabular}\end{sideways}} % multi-line sideways, centered

% ---------
% FUNCTIONS
% ---------
\newcommand{\func}[1]{\textsc{#1}} % function names for programming

% \newcommand{\G}[1]{\Gamma(#1)} % gamma function
\newcommand{\GQ}[2]{Q_{#1}(#2)} % regularized (upper) incomplete gamma function
\newcommand{\GP}[2]{P_{#1}(#2)} % regularized (lower) incomplete gamma function
\newcommand{\B}[3]{B\if*#1\else_{#1}\fi(#2,#3)} % (incomplete) beta function
\newcommand{\I}[3]{I\if*#1\else_{#1}\fi(#2,#3)} % regularized incomplete beta function
\newcommand{\Digamma}[1]{\Psi(#1)} % digamma function
\newcommand{\harmonic}[1]{H_{#1}} % harmonic number

% (mod ...), tight spacing
\makeatletter
\def\imod#1{\allowbreak\mkern10mu({\operator@font mod}\,\,#1)}
\makeatother

% ------
% BIG-OH
% ------
\newcommand{\bigO}[1]{O\!\left(#1\right)} % at most
\newcommand{\bigOn}[1]{O(#1)} % at most
\newcommand{\bigObig}[1]{O\bigl(#1\bigr)} % at most
\newcommand{\bigOmega}[1]{\Omega\!\left(#1\right)} % at least
\newcommand{\bigOmegan}[1]{\Omega(#1)} % at least
\newcommand{\bigTheta}[1]{\Theta\!\left(#1\right)} % at least and at most
\newcommand{\smallo}[1]{o\!\left(#1\right)} % asymptotically negligible (ratio f(x)/g(x)-->0)

%% -----------
%% CONVERGENCE
%% -----------
\newcommand{\toas}{\xrightarrow{\text{a.s.}}}

% -----------
% INTEGRATION
% -----------
\newcommand{\dd}{\; \mathrm{d}} % correct spacing and formating


% ------------
% ENVIRONMENTS
% ------------
%\newtheorem{lemma}{Lemma}
%\newtheorem{theorem}{Theorem}
%\newtheorem{proposition}{Proposition}
%\newtheorem{corollary}{Corollary}

% ------
% SPACES
% ------
\newlength\hspaceoflen
\newcommand\hspaceof[1]{\settowidth\hspaceoflen{#1}\hspace\hspaceoflen}

%% vertically centered
\newcommand{\vcentered}[1]{\begingroup\setbox0=\hbox{#1}\parbox{\wd0}{\box0}\endgroup}

% ----------------
% VECTOR VARIABLES
% ----------------
\newcommand\vect[1]{{\boldsymbol{#1}}}
\newcommand\va{\vect{a}}
\newcommand\vb{\vect{b}}
\newcommand\vc{\vect{c}}
\newcommand\vd{\vect{d}}
\newcommand\ve{\vect{e}}
\newcommand\vf{\vect{f}}
\newcommand\vg{\vect{g}}
\newcommand\vh{\vect{h}}
\newcommand\vi{\vect{i}}
\newcommand\vj{\vect{j}}
\newcommand\vk{\vect{k}}
\newcommand\vl{\vect{l}}
\newcommand\vm{\vect{m}}
\newcommand\vn{\vect{n}}
\newcommand\vo{\vect{o}}
\newcommand\vp{\vect{p}}
\newcommand\vq{\vect{q}}
\newcommand\vr{\vect{r}}
\newcommand\vs{\vect{s}}
\newcommand\vt{\vect{t}}
\newcommand\vu{\vect{u}}
\newcommand\vv{\vect{v}}
\newcommand\vw{\vect{w}}
\newcommand\vx{\vect{x}}
\newcommand\vy{\vect{y}}
\newcommand\vz{\vect{z}}
\newcommand\vzero{\vect{0}}
\newcommand\vone{\vect{1}}

\newcommand\valpha{\vect{\alpha}}
\newcommand\vbeta{\vect{\beta}}
\newcommand\veps{\vect{\epsilon}}
\newcommand\vdelta{\vect{\delta}}
\newcommand\veta{\vect{\eta}}
\newcommand\vgamma{\vect{\gamma}}
\newcommand\vtau{\vect{\tau}}
\newcommand\vtheta{\vect{\theta}}
\newcommand\vmu{\vect{\mu}}
\newcommand\vsigma{\vect{\sigma}}
\newcommand\vpi{\vect{\pi}}
\newcommand\vlambda{\vect{\lambda}}

% ----------------
% MATRIX VARIABLES
% ----------------
\newcommand\mA{\vect{A}}
\newcommand\mB{\vect{B}}
\newcommand\mC{\vect{C}}
\newcommand\mD{\vect{D}}
\newcommand\mE{\vect{E}}
\newcommand\mF{\vect{F}}
\newcommand\mG{\vect{G}}
\newcommand\mH{\vect{H}}
\newcommand\mI{\vect{I}}
\newcommand\mJ{\vect{J}}
\newcommand\mK{\vect{K}}
\newcommand\mL{\vect{L}}
\newcommand\mM{\vect{M}}
\newcommand\mN{\vect{N}}
\newcommand\mO{\vect{O}}
\newcommand\mP{\vect{P}}
\newcommand\mQ{\vect{Q}}
\newcommand\mR{\vect{R}}
\newcommand\mS{\vect{S}}
\newcommand\mT{\vect{T}}
\newcommand\mU{\vect{U}}
\newcommand\mV{\vect{V}}
\newcommand\mW{\vect{W}}
\newcommand\mX{\vect{X}}
\newcommand\mY{\vect{Y}}
\newcommand\mZ{\vect{Z}}
\newcommand\mzero{\vect{0}}

\newcommand{\mEps}{{\ensuremath{\vect{\Epsilon}}}}
\newcommand{\mSigma}{{\ensuremath{\vect{\Sigma}}}}
\newcommand{\mLambda}{{\ensuremath{\vect{\Lambda}}}}
\newcommand{\mPsi}{{\ensuremath{\vect{\Psi}}}}

% ------------------
% BLACKBOARD LETTERS
% ------------------
\newcommand\bA{\mathbb{A}}
\newcommand\bB{\mathbb{B}}
\newcommand\bC{\mathbb{C}} % set of complex numbers
\newcommand\bD{\mathbb{D}}
\newcommand\bE{\mathbb{E}}
\newcommand\bF{\mathbb{F}}
\newcommand\bG{\mathbb{G}}
\newcommand\bH{\mathbb{H}}
\newcommand\bI{\mathbb{I}}
\newcommand\bJ{\mathbb{J}}
\newcommand\bK{\mathbb{K}}
\newcommand\bL{\mathbb{L}}
\newcommand\bM{\mathbb{M}}
\newcommand\bN{\mathbb{N}} % set of positive integers
\newcommand\bO{\mathbb{O}}
\newcommand\bP{\mathbb{P}}
\newcommand\bQ{\mathbb{Q}} % set of rationals
\newcommand\bR{\mathbb{R}} % set of reals
\newcommand\bS{\mathbb{S}}
\newcommand\bT{\mathbb{T}}
\newcommand\bU{\mathbb{U}}
\newcommand\bV{\mathbb{V}}
\newcommand\bW{\mathbb{W}}
\newcommand\bX{\mathbb{X}}
\newcommand\bY{\mathbb{Y}}
\newcommand\bZ{\mathbb{Z}} % set of all integers

% -------------
% FANCY LETTERS
% -------------

% requires mathrsfs package
\newcommand\xA{\mathscr{A}}
\newcommand\xB{\mathscr{B}}
\newcommand\xC{\mathscr{C}}
\newcommand\xD{\mathscr{D}}
\newcommand\xE{\mathscr{E}}
\newcommand\xF{\mathscr{F}}
\newcommand\xG{\mathscr{G}}
\newcommand\xH{\mathscr{H}}
\newcommand\xI{\mathscr{I}}
\newcommand\xJ{\mathscr{J}}
\newcommand\xK{\mathscr{K}}
\newcommand\xL{\mathscr{L}}
\newcommand\xM{\mathscr{M}}
\newcommand\xN{\mathscr{N}}
\newcommand\xO{\mathscr{O}}
\newcommand\xP{\mathscr{P}}
\newcommand\xQ{\mathscr{Q}}
\newcommand\xR{\mathscr{R}}
\newcommand\xS{\mathscr{S}}
\newcommand\xT{\mathscr{T}}
\newcommand\xU{\mathscr{U}}
\newcommand\xV{\mathscr{V}}
\newcommand\xW{\mathscr{W}}
\newcommand\xX{\mathscr{X}}
\newcommand\xY{\mathscr{Y}}
\newcommand\xZ{\mathscr{Z}}

% --------------------
% CALLIGRAPHIC LETTERS
% --------------------
\DeclareMathAlphabet{\mathcal}{OMS}{cmsy}{m}{n}
\newcommand\cA{\mathcal{A}}
\newcommand\cB{\mathcal{B}}
\newcommand\cC{\mathcal{C}}
\newcommand\cD{\mathcal{D}}
\newcommand\cE{\mathcal{E}}
\newcommand\cF{\mathcal{F}}
\newcommand\cG{\mathcal{G}}
\newcommand\cH{\mathcal{H}}
\newcommand\cI{\mathcal{I}}
\newcommand\cJ{\mathcal{J}}
\newcommand\cK{\mathcal{K}}
\newcommand\cL{\mathcal{L}}
\newcommand\cM{\mathcal{M}}
\newcommand\cN{\mathcal{N}}
\newcommand\cO{\mathcal{O}}
\newcommand\cP{\mathcal{P}}
\newcommand\cQ{\mathcal{Q}}
\newcommand\cR{\mathcal{R}}
\newcommand\cS{\mathcal{S}}
\newcommand\cT{\mathcal{T}}
\newcommand\cU{\mathcal{U}}
\newcommand\cV{\mathcal{V}}
\newcommand\cW{\mathcal{W}}
\newcommand\cX{\mathcal{X}}
\newcommand\cY{\mathcal{Y}}
\newcommand\cZ{\mathcal{Z}}

% -------------------------
% BOLD CALLIGRAPHIC LETTERS
% -------------------------
\DeclareMathAlphabet\mathbfcal{OMS}{cmsy}{b}{n}
\newcommand\tA{\mathbfcal{A}}
\newcommand\tB{\mathbfcal{B}}
\newcommand\tC{\mathbfcal{C}}
\newcommand\tD{\mathbfcal{D}}
\newcommand\tE{\mathbfcal{E}}
\newcommand\tF{\mathbfcal{F}}
\newcommand\tG{\mathbfcal{G}}
\newcommand\tH{\mathbfcal{H}}
\newcommand\tI{\mathbfcal{I}}
\newcommand\tJ{\mathbfcal{J}}
\newcommand\tK{\mathbfcal{K}}
\newcommand\tL{\mathbfcal{L}}
\newcommand\tM{\mathbfcal{M}}
\newcommand\tN{\mathbfcal{N}}
\newcommand\tO{\mathbfcal{O}}
\newcommand\tP{\mathbfcal{P}}
\newcommand\tQ{\mathbfcal{Q}}
\newcommand\tR{\mathbfcal{R}}
\newcommand\tS{\mathbfcal{S}}
\newcommand\tT{\mathbfcal{T}}
\newcommand\tU{\mathbfcal{U}}
\newcommand\tV{\mathbfcal{V}}
\newcommand\tW{\mathbfcal{W}}
\newcommand\tX{\mathbfcal{X}}
\newcommand\tY{\mathbfcal{Y}}
\newcommand\tZ{\mathbfcal{Z}}



% -----------------
% LETTERS WITH HATS
% -----------------

% use amsxtra package!

\newcommand\Ahat{{\hat A}}
\newcommand\Bhat{{\hat B}}
\newcommand\Chat{{\hat C}}
\newcommand\Dhat{{\hat D}}
\newcommand\Ehat{{\hat E}}
\newcommand\Fhat{{\hat F}}
\newcommand\Ghat{{\hat G}}
\newcommand\Hhat{{\hat H}}
\newcommand\Ihat{{\hat I}}
\newcommand\Jhat{{\hat J}}
\newcommand\Khat{{\hat K}}
\newcommand\Lhat{{\hat L}}
\newcommand\Mhat{{\hat M}}
\newcommand\Nhat{{\hat N}}
\newcommand\Ohat{{\hat O}}
\newcommand\Phat{{\hat P}}
\newcommand\Qhat{{\hat Q}}
\newcommand\Rhat{{\hat R}}
\newcommand\Shat{{\hat S}}
\newcommand\That{{\hat T}}
\newcommand\Uhat{{\hat U}}
\newcommand\Vhat{{\hat V}}
\newcommand\What{{\hat W}}
\newcommand\Xhat{{\hat X}}
\newcommand\Yhat{{\hat Y}}
\newcommand\Zhat{{\hat Z}}

\newcommand\ahat{{\hat a}}
\newcommand\bhat{{\hat b}}
\newcommand\chat{{\hat c}}
\newcommand\dhat{{\hat d}}
\newcommand\ehat{{\hat e}}
\newcommand\fhat{{\hat f}}
\newcommand\ghat{{\hat g}}
\newcommand\hhat{{\hat h}}
\newcommand\ihat{{\hat i}}
\newcommand\jhat{{\hat j}}
\newcommand\khat{{\hat k}}
\newcommand\lhat{{\hat l}}
\newcommand\mhat{{\hat m}}
\newcommand\nhat{{\hat n}}
\newcommand\ohat{{\hat o}}
\newcommand\phat{{\hat p}}
\newcommand\qhat{{\hat q}}
\newcommand\rhat{{\hat r}}
\newcommand\shat{{\hat s}}
\newcommand\that{{\hat t}}
\newcommand\uhat{{\hat u}}
\newcommand\vhat{{\hat v}}
\newcommand\what{{\hat w}}
\newcommand\xhat{{\hat x}}
\newcommand\yhat{{\hat y}}
\newcommand\zhat{{\hat z}}

\newcommand\rhohat{{\hat\rho}}

% -----------------
% LETTERS WITH BARS
% -----------------

\accentedsymbol\Abar{{\bar A}}
\accentedsymbol\Bbar{{\bar B}}
\accentedsymbol\Cbar{{\bar C}}
\accentedsymbol\Dbar{{\bar D}}
\accentedsymbol\Ebar{{\bar E}}
\accentedsymbol\Fbar{{\bar F}}
\accentedsymbol\Gbar{{\bar G}}
\accentedsymbol\Hbar{{\bar H}}
\accentedsymbol\Ibar{{\bar I}}
\accentedsymbol\Jbar{{\bar J}}
\accentedsymbol\Kbar{{\bar K}}
\accentedsymbol\Lbar{{\bar L}}
\accentedsymbol\Mbar{{\bar M}}
\accentedsymbol\Nbar{{\bar N}}
\accentedsymbol\Obar{{\bar O}}
\accentedsymbol\Pbar{{\bar P}}
\accentedsymbol\Qbar{{\bar Q}}
\accentedsymbol\Rbar{{\bar R}}
\accentedsymbol\Sbar{{\bar S}}
\accentedsymbol\Tbar{{\bar T}}
\accentedsymbol\Ubar{{\bar U}}
\accentedsymbol\Vbar{{\bar V}}
\accentedsymbol\Wbar{{\bar W}}
\accentedsymbol\Xbar{{\bar X}}
\accentedsymbol\Ybar{{\bar Y}}
\accentedsymbol\Zbar{{\bar Z}}

\accentedsymbol\abar{{\bar a}}
\accentedsymbol\bbar{{\bar b}}
\accentedsymbol\cbar{{\bar c}}
\accentedsymbol\dbar{{\bar d}}
\accentedsymbol\ebar{{\bar e}}
\accentedsymbol\fbar{{\bar f}}
\accentedsymbol\gbar{{\bar g}}
\makeatletter
\@ifundefined{hbar}{}{
        \let\oldhbar\hbar % we are going to overwrite an existing command; keep the old version
        \let\hbar\@undefined
}
\makeatother
\accentedsymbol\hbar{{\bar h}}
\accentedsymbol\ibar{{\bar i}}
\accentedsymbol\jbar{{\bar j}}
\accentedsymbol\kbar{{\bar k}}
\accentedsymbol\lbar{{\bar l}}
\accentedsymbol\mbar{{\bar m}}
\accentedsymbol\nbar{{\bar n}}
\makeatletter
\@ifundefined{obar}{}{
        \let\oldobar\obar % we are going to overwrite an existing command; keep the old version
        \let\obar\@undefined
}
\makeatother
\accentedsymbol{\obar}{{\bar o}}
\accentedsymbol\pbar{{\bar p}}
\accentedsymbol\qbar{{\bar q}}
\accentedsymbol\rbar{{\bar r}}
\accentedsymbol\sbar{{\bar s}}
\accentedsymbol\tbar{{\bar t}}
\accentedsymbol\ubar{{\bar u}}
\accentedsymbol\vbar{{\bar v}}
\accentedsymbol\wbar{{\bar w}}
\accentedsymbol\xbar{{\bar x}}
\accentedsymbol\ybar{{\bar y}}
\accentedsymbol\zbar{{\bar z}}

% -------------
% GREEK LETTERS
% -------------
\newcommand\eps{\epsilon}


% ---------------------------------
% MATRIX/VECTOR VARIABLES WITH HATS
% ---------------------------------

\accentedsymbol\mAhat{{\hat\mA}}
\accentedsymbol\mBhat{{\hat\mB}}
\accentedsymbol\mChat{{\hat\mC}}
\accentedsymbol\mDhat{{\hat\mD}}
\accentedsymbol\mEhat{{\hat\mE}}
\accentedsymbol\mFhat{{\hat\mF}}
\accentedsymbol\mGhat{{\hat\mG}}
\accentedsymbol\mHhat{{\hat\mH}}
\accentedsymbol\mIhat{{\hat\mI}}
\accentedsymbol\mJhat{{\hat\mJ}}
\accentedsymbol\mKhat{{\hat\mK}}
\accentedsymbol\mLhat{{\hat\mL}}
\accentedsymbol\mMhat{{\hat\mM}}
\accentedsymbol\mNhat{{\hat\mN}}
\accentedsymbol\mOhat{{\hat\mO}}
\accentedsymbol\mPhat{{\hat\mP}}
\accentedsymbol\mQhat{{\hat\mQ}}
\accentedsymbol\mRhat{{\hat\mR}}
\accentedsymbol\mShat{{\hat\mS}}
\accentedsymbol\mThat{{\hat\mT}}
\accentedsymbol\mUhat{{\hat\mU}}
\accentedsymbol\mVhat{{\hat\mV}}
\accentedsymbol\mWhat{{\hat\mW}}
\accentedsymbol\mXhat{{\hat\mX}}
\accentedsymbol\mYhat{{\hat\mY}}
\accentedsymbol\mZhat{{\hat\mZ}}

\accentedsymbol\vahat{{\hat\va}}
\accentedsymbol\vbhat{{\hat\vb}}
\accentedsymbol\vchat{{\hat\vc}}
\accentedsymbol\vdhat{{\hat\vd}}
\accentedsymbol\vehat{{\hat\ve}}
\accentedsymbol\vfhat{{\hat\vf}}
\accentedsymbol\vghat{{\hat\vg}}
\accentedsymbol\vhhat{{\hat\vh}}
\accentedsymbol\vihat{{\hat\vi}}
\accentedsymbol\vjhat{{\hat\vj}}
\accentedsymbol\vkhat{{\hat\vk}}
\accentedsymbol\vlhat{{\hat\vl}}
\accentedsymbol\vmhat{{\hat\vm}}
\accentedsymbol\vnhat{{\hat\vn}}
\accentedsymbol\vohat{{\hat\vo}}
\accentedsymbol\vphat{{\hat\vp}}
\accentedsymbol\vqhat{{\hat\vq}}
\accentedsymbol\vrhat{{\hat\vr}}
\accentedsymbol\vshat{{\hat\vs}}
\accentedsymbol\vthat{{\hat\vt}}
\accentedsymbol\vuhat{{\hat\vu}}
\accentedsymbol\vvhat{{\hat\vv}}
\accentedsymbol\vwhat{{\hat\vw}}
\accentedsymbol\vxhat{{\hat\vx}}
\accentedsymbol\vyhat{{\hat\vy}}
\accentedsymbol\vzhat{{\hat\vz}}

==> main/xkeyval.tex <==
%%
%% This is file `xkeyval.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xkeyval.dtx  (with options: `xkvtex')
%% 
%% ---------------------------------------
%% Copyright (C) 2004-2014 Hendri Adriaens
%% ---------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2003/12/01 or later.
%%
%% This work has the LPPL maintenance status "maintained".
%%
%% This Current Maintainer of this work is Hendri Adriaens.
%%
%% This work consists of the file xkeyval.dtx and derived files
%% keyval.tex, xkvtxhdr.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, xkvutils.tex, pst-xkey.tex, pst-xkey.sty, xkveca.cls,
%% xkvecb.cls, xkvesa.sty, xkvesb.sty, xkvesc.sty, xkvex1.tex,
%% xkvex2.tex, xkvex3.tex and xkvex4.tex.
%%
%% The following files constitute the xkeyval bundle and must be
%% distributed as a whole: readme, xkeyval.pdf, keyval.tex,
%% pst-xkey.sty, pst-xkey.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, xkvtxhdr.tex, xkvutils.tex, pst-xkey.dtx and xkeyval.dtx.
%%
\csname XKeyValLoaded\endcsname
\let\XKeyValLoaded\endinput
\edef\XKVcatcodes{%
  \catcode`\noexpand\@\the\catcode`\@\relax
  \catcode`\noexpand\=\the\catcode`\=\relax
  \catcode`\noexpand\,\the\catcode`\,\relax
  \catcode`\noexpand\:\the\catcode`\:\relax
  \let\noexpand\XKVcatcodes\relax
}
\catcode`\@11\relax
\catcode`\=12\relax
\catcode`\,12\relax
\catcode`\:12\relax
\input xkvutils
\newcount\XKV@depth
\newif\ifXKV@st
\newif\ifXKV@sg
\newif\ifXKV@pl
\newif\ifXKV@knf
\newif\ifXKV@rkv
\newif\ifXKV@inpox
\newif\ifXKV@preset
\let\XKV@rm\@empty
\ifx\ProvidesFile\@undefined
  \message{2014/12/03 v2.7a key=value parser (HA)}
  \input xkvtxhdr
\else
  \ProvidesFile{xkeyval.tex}[2014/12/03 v2.7a key=value parser (HA)]
  \@addtofilelist{xkeyval.tex}
\fi
\def\XKV@warn#1{\message{xkeyval warning: #1}}
\def\XKV@err#1{\errmessage{xkeyval error: #1}}
\def\KV@errx{\XKV@err}
\let\KV@err\KV@errx
\def\XKV@ifstar#1{\@ifnextcharacter*{\@firstoftwo{#1}}}
\def\XKV@ifplus#1{\@ifnextcharacter+{\@firstoftwo{#1}}}
\def\XKV@makepf#1{%
  \KV@@sp@def\XKV@prefix{#1}%
  \def\XKV@resa{XKV}%
  \ifx\XKV@prefix\XKV@resa
    \XKV@err{`XKV' prefix is not allowed}%
    \let\XKV@prefix\@empty
  \else
    \edef\XKV@prefix{\ifx\XKV@prefix\@empty\else\XKV@prefix @\fi}%
  \fi
}
\def\XKV@makehd#1{%
  \expandafter\KV@@sp@def\expandafter\XKV@header\expandafter{#1}%
  \edef\XKV@header{%
    \XKV@prefix\ifx\XKV@header\@empty\else\XKV@header @\fi
  }%
}
\def\XKV@srstate#1#2{%
  \ifx\@empty#2\@empty\advance\XKV@depth\@ne\fi
  \XKV@for@n{XKV@prefix,XKV@fams,XKV@tkey,XKV@na,%
    ifXKV@st,ifXKV@pl,ifXKV@knf,CurrentOption}\XKV@resa{%
    \expandafter\let\csname\XKV@resa#1\expandafter
      \endcsname\csname\XKV@resa#2\endcsname
  }%
  \ifx\@empty#1\@empty\advance\XKV@depth\m@ne\fi
}
\def\XKV@testopta#1{%
  \XKV@ifstar{\XKV@sttrue\XKV@t@stopta{#1}}%
    {\XKV@stfalse\XKV@t@stopta{#1}}%
}
\def\XKV@t@stopta#1{\XKV@ifplus{\XKV@pltrue#1}{\XKV@plfalse#1}}
\def\XKV@testoptb#1{\@testopt{\XKV@t@stoptb#1}{KV}}
\def\XKV@t@stoptb#1[#2]#3{%
  \XKV@makepf{#2}%
  \XKV@makehd{#3}%
  \KV@@sp@def\XKV@tfam{#3}%
  #1%
}
\def\XKV@testoptc#1{\@testopt{\XKV@t@stoptc#1}{KV}}
\def\XKV@t@stoptc#1[#2]#3{%
  \XKV@makepf{#2}%
  \XKV@checksanitizeb{#3}\XKV@fams
  \expandafter\XKV@sp@deflist\expandafter
    \XKV@fams\expandafter{\XKV@fams}%
  \@testopt#1{}%
}
\def\XKV@testoptd#1#2{%
  \XKV@testoptb{%
    \edef\XKV@tempa{#2\XKV@header}%
    \def\XKV@tempb{\@testopt{\XKV@t@stoptd#1}}%
    \expandafter\XKV@tempb\expandafter{\XKV@tempa}%
  }%
}
\def\XKV@t@stoptd#1[#2]#3{%
  \@ifnextchar[{\XKV@sttrue#1{#2}{#3}}{\XKV@stfalse#1{#2}{#3}[]}%
}
\def\XKV@ifcmd#1#2#3{%
  \def\XKV@@ifcmd##1#2##2##3\@nil##4{%
    \def##4{##2}\ifx##4\@nnil
      \def##4{##1}\expandafter\@secondoftwo
    \else
      \expandafter\@firstoftwo
    \fi
  }%
  \XKV@@ifcmd#1#2{\@nil}\@nil#3%
}
\def\XKV@getkeyname#1#2{\expandafter\XKV@g@tkeyname#1=\@nil#2}
\long\def\XKV@g@tkeyname#1=#2\@nil#3{%
  \XKV@ifcmd{#1}\savevalue#3{\XKV@rkvtrue\XKV@sgfalse}{%
    \XKV@ifcmd{#1}\gsavevalue#3%
      {\XKV@rkvtrue\XKV@sgtrue}{\XKV@rkvfalse\XKV@sgfalse}%
  }%
}
\def\XKV@getsg#1#2{%
  \expandafter\XKV@ifcmd\expandafter{#1}\global#2\XKV@sgtrue\XKV@sgfalse
}
\def\XKV@define@default#1#2{%
  \expandafter\def\csname\XKV@header#1@default\expandafter
    \endcsname\expandafter{\csname\XKV@header#1\endcsname{#2}}%
}
\def\define@key{\XKV@testoptb\XKV@define@key}
\def\XKV@define@key#1{%
  \@ifnextchar[{\XKV@d@fine@k@y{#1}}{%
    \long\expandafter\def\csname\XKV@header#1\endcsname####1%
  }%
}
\def\XKV@d@fine@k@y#1[#2]{%
  \XKV@define@default{#1}{#2}%
  \expandafter\def\csname\XKV@header#1\endcsname##1%
}
\def\define@cmdkey{\XKV@testoptd\XKV@define@cmdkey{cmd}}
\def\XKV@define@cmdkey#1#2[#3]#4{%
  \ifXKV@st\XKV@define@default{#2}{#3}\fi
  \def\XKV@tempa{\expandafter\def\csname\XKV@header#2\endcsname####1}%
  \begingroup\expandafter\endgroup\expandafter\XKV@tempa\expandafter
    {\expandafter\def\csname#1#2\endcsname{##1}#4}%
}
\def\define@cmdkeys{\XKV@testoptd\XKV@define@cmdkeys{cmd}}
\def\XKV@define@cmdkeys#1#2[#3]{%
  \XKV@sp@deflist\XKV@tempa{#2}%
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \edef\XKV@tempa{\noexpand\XKV@define@cmdkey{#1}{\XKV@tempa}}%
    \XKV@tempa[#3]{}%
  }%
}
\def\define@choicekey{\XKV@testopta{\XKV@testoptb\XKV@define@choicekey}}
\def\XKV@define@choicekey#1{\@testopt{\XKV@d@fine@choicekey{#1}}{}}
\def\XKV@d@fine@choicekey#1[#2]#3{%
  \toks@{#2}%
  \XKV@sp@deflist\XKV@tempa{#3}\XKV@toks\expandafter{\XKV@tempa}%
  \@ifnextchar[{\XKV@d@fine@ch@icekey{#1}}{\XKV@d@fine@ch@ic@key{#1}}%
}
\def\XKV@d@fine@ch@icekey#1[#2]{%
  \XKV@define@default{#1}{#2}%
  \XKV@d@fine@ch@ic@key{#1}%
}
\def\XKV@d@fine@ch@ic@key#1{%
  \ifXKV@pl\XKV@afterelsefi
    \expandafter\XKV@d@f@ne@ch@ic@k@y
  \else\XKV@afterfi
    \expandafter\XKV@d@f@ne@ch@ic@key
  \fi
  \csname\XKV@header#1\endcsname
}
\def\XKV@d@f@ne@ch@ic@key#1#2{\XKV@d@f@n@@ch@ic@k@y#1{{#2}}}
\def\XKV@d@f@ne@ch@ic@k@y#1#2#3{\XKV@d@f@n@@ch@ic@k@y#1{{#2}{#3}}}
\def\XKV@d@f@n@@ch@ic@k@y#1#2{%
  \edef#1##1{%
    \ifXKV@st\noexpand\XKV@sttrue\else\noexpand\XKV@stfalse\fi
    \ifXKV@pl\noexpand\XKV@pltrue\else\noexpand\XKV@plfalse\fi
    \noexpand\XKV@checkchoice[\the\toks@]{##1}{\the\XKV@toks}%
  }%
  \def\XKV@tempa{\def#1####1}%
  \expandafter\XKV@tempa\expandafter{#1{##1}#2}%
}
\def\define@boolkey{\XKV@t@stopta{\XKV@testoptd\XKV@define@boolkey{}}}
\def\XKV@define@boolkey#1#2[#3]{%
  \ifXKV@pl\XKV@afterelsefi
    \expandafter\XKV@d@f@ne@boolkey
  \else\XKV@afterfi
    \expandafter\XKV@d@fine@boolkey
  \fi
  \csname\XKV@header#2\endcsname{#2}{#1#2}{#3}%
}
\def\XKV@d@fine@boolkey#1#2#3#4#5{%
  \XKV@d@f@ne@b@olkey#1{#2}{#3}{#4}%
    {{\csname#3\XKV@resa\endcsname#5}}%
}
\def\XKV@d@f@ne@boolkey#1#2#3#4#5#6{%
  \XKV@d@f@ne@b@olkey#1{#2}{#3}{#4}%
    {{\csname#3\XKV@resa\endcsname#5}{#6}}%
}
\def\XKV@d@f@ne@b@olkey#1#2#3#4#5{%
  \expandafter\newif\csname if#3\endcsname
  \ifXKV@st\XKV@define@default{#2}{#4}\fi
  \ifXKV@pl
    \def#1##1{\XKV@pltrue\XKV@sttrue
      \XKV@checkchoice[\XKV@resa]{##1}{true,false}#5%
    }%
  \else
    \def#1##1{\XKV@plfalse\XKV@sttrue
      \XKV@checkchoice[\XKV@resa]{##1}{true,false}#5%
    }%
  \fi
}
\def\define@boolkeys{\XKV@plfalse\XKV@testoptd\XKV@define@boolkeys{}}
\def\XKV@define@boolkeys#1#2[#3]{%
  \XKV@sp@deflist\XKV@tempa{#2}%
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \expandafter\XKV@d@fine@boolkeys\expandafter{\XKV@tempa}{#1}{#3}%
  }%
}
\def\XKV@d@fine@boolkeys#1#2#3{%
  \expandafter\XKV@d@f@ne@b@olkey\csname\XKV@header#1\endcsname
    {#1}{#2#1}{#3}{{\csname#2#1\XKV@resa\endcsname}}%
}
\def\XKV@cc{\XKV@testopta{\@testopt\XKV@checkchoice{}}}
\def\XKV@checkchoice[#1]#2#3{%
  \def\XKV@tempa{#1}%
  \ifXKV@st\lowercase{\fi
  \ifx\XKV@tempa\@empty
    \def\XKV@tempa{\XKV@ch@ckch@ice\@nil{#2}{#3}}%
  \else
    \def\XKV@tempa{\XKV@ch@ckchoice#1\@nil{#2}{#3}}%
  \fi
  \ifXKV@st}\fi\XKV@tempa
}
\def\XKV@ch@ckchoice#1#2\@nil#3#4{%
  \def\XKV@tempa{#2}%
  \ifx\XKV@tempa\@empty\XKV@afterelsefi
    \XKV@ch@ckch@ice#1{#3}{#4}%
  \else\XKV@afterfi
    \XKV@@ch@ckchoice#1#2{#3}{#4}%
  \fi
}
\def\XKV@ch@ckch@ice#1#2#3{%
  \def\XKV@tempa{#1}%
  \ifx\XKV@tempa\@nnil\let\XKV@tempa\@empty\else
    \def\XKV@tempa{\def#1{#2}}%
  \fi
  \in@{,#2,}{,#3,}%
  \ifin@
    \ifXKV@pl
      \XKV@addtomacro@n\XKV@tempa\@firstoftwo
    \else
      \XKV@addtomacro@n\XKV@tempa\@firstofone
    \fi
  \else
    \ifXKV@pl
      \XKV@addtomacro@n\XKV@tempa\@secondoftwo
    \else
      \XKV@toks{#2}%
      \XKV@err{value `\the\XKV@toks' is not allowed}%
      \XKV@addtomacro@n\XKV@tempa\@gobble
    \fi
  \fi
  \XKV@tempa
}
\def\XKV@@ch@ckchoice#1#2#3#4{%
  \edef\XKV@tempa{\the\count@}\count@\z@
  \def\XKV@tempb{#3}%
  \def\XKV@tempc##1,{%
    \def#1{##1}%
    \ifx#1\@nnil
      \def#1{#3}\def#2{-1}\count@\XKV@tempa
      \ifXKV@pl
        \let\XKV@tempd\@secondoftwo
      \else
        \XKV@toks{#3}%
        \XKV@err{value `\the\XKV@toks' is not allowed}%
        \let\XKV@tempd\@gobble
      \fi
    \else
      \ifx#1\XKV@tempb
        \edef#2{\the\count@}\count@\XKV@tempa
        \ifXKV@pl
          \let\XKV@tempd\XKV@@ch@ckch@ice
        \else
          \let\XKV@tempd\XKV@@ch@ckch@ic@
        \fi
      \else
        \advance\count@\@ne
        \let\XKV@tempd\XKV@tempc
      \fi
    \fi
    \XKV@tempd
  }%
  \XKV@tempc#4,\@nil,%
}
\def\XKV@@ch@ckch@ice#1\@nil,{\@firstoftwo}
\def\XKV@@ch@ckch@ic@#1\@nil,{\@firstofone}
\def\key@ifundefined{\@testopt\XKV@key@ifundefined{KV}}
\def\XKV@key@ifundefined[#1]#2{%
  \XKV@makepf{#1}%
  \XKV@checksanitizeb{#2}\XKV@fams
  \expandafter\XKV@sp@deflist\expandafter
    \XKV@fams\expandafter{\XKV@fams}%
  \XKV@key@if@ndefined
}
\def\XKV@key@if@ndefined#1{%
  \XKV@knftrue
  \KV@@sp@def\XKV@tkey{#1}%
  \XKV@whilist\XKV@fams\XKV@tfam\ifXKV@knf\fi{%
    \XKV@makehd\XKV@tfam
    \XKV@ifundefined{\XKV@header\XKV@tkey}{}{\XKV@knffalse}%
  }%
  \ifXKV@knf
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
}
\def\disable@keys{\XKV@testoptb\XKV@disable@keys}
\def\XKV@disable@keys#1{%
  \XKV@checksanitizeb{#1}\XKV@tempa
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \XKV@ifundefined{\XKV@header\XKV@tempa}{%
      \XKV@err{key `\XKV@tempa' undefined}%
    }{%
      \edef\XKV@tempb{%
        \noexpand\XKV@warn{key `\XKV@tempa' has been disabled}%
      }%
      \XKV@ifundefined{\XKV@header\XKV@tempa @default}{%
        \edef\XKV@tempc{\noexpand\XKV@define@key{\XKV@tempa}}%
      }{%
        \edef\XKV@tempc{\noexpand\XKV@define@key{\XKV@tempa}[]}%
      }%
      \expandafter\XKV@tempc\expandafter{\XKV@tempb}%
    }%
  }%
}
\def\presetkeys{\XKV@stfalse\XKV@testoptb\XKV@presetkeys}
\def\gpresetkeys{\XKV@sttrue\XKV@testoptb\XKV@presetkeys}
\def\XKV@presetkeys#1#2{%
  \XKV@pr@setkeys{#1}{preseth}%
  \XKV@pr@setkeys{#2}{presett}%
}
\def\XKV@pr@setkeys#1#2{%
  \XKV@ifundefined{XKV@\XKV@header#2}{%
    \XKV@checksanitizea{#1}\XKV@tempa
    \ifXKV@st\expandafter\global\fi\expandafter\def\csname
      XKV@\XKV@header#2\expandafter\endcsname\expandafter{\XKV@tempa}%
  }{%
    \expandafter\XKV@merge\csname XKV@\XKV@header
      #2\endcsname{#1}\XKV@getkeyname
  }%
}
\def\delpresetkeys{\XKV@stfalse\XKV@testoptb\XKV@delpresetkeys}
\def\gdelpresetkeys{\XKV@sttrue\XKV@testoptb\XKV@delpresetkeys}
\def\XKV@delpresetkeys#1#2{%
  \XKV@d@lpresetkeys{#1}{preseth}%
  \XKV@d@lpresetkeys{#2}{presett}%
}
\def\XKV@d@lpresetkeys#1#2{%
  \XKV@ifundefined{XKV@\XKV@header#2}{%
    \XKV@err{no presets defined for `\XKV@header'}%
  }{%
    \expandafter\XKV@delete\csname XKV@\XKV@header
      #2\endcsname{#1}\XKV@getkeyname
  }%
}
\def\unpresetkeys{\XKV@stfalse\XKV@testoptb\XKV@unpresetkeys}
\def\gunpresetkeys{\XKV@sttrue\XKV@testoptb\XKV@unpresetkeys}
\def\XKV@unpresetkeys{%
  \XKV@ifundefined{XKV@\XKV@header preseth}{%
    \XKV@err{no presets defined for `\XKV@header'}%
  }{%
    \ifXKV@st\expandafter\global\fi\expandafter\let
      \csname XKV@\XKV@header preseth\endcsname\@undefined
    \ifXKV@st\expandafter\global\fi\expandafter\let
      \csname XKV@\XKV@header presett\endcsname\@undefined
  }%
}
\def\savekeys{\XKV@stfalse\XKV@testoptb\XKV@savekeys}
\def\gsavekeys{\XKV@sttrue\XKV@testoptb\XKV@savekeys}
\def\XKV@savekeys#1{%
  \XKV@ifundefined{XKV@\XKV@header save}{%
    \XKV@checksanitizeb{#1}\XKV@tempa
    \ifXKV@st\expandafter\global\fi\expandafter\def\csname XKV@%
      \XKV@header save\expandafter\endcsname\expandafter{\XKV@tempa}%
  }{%
    \expandafter\XKV@merge\csname XKV@\XKV@header
      save\endcsname{#1}\XKV@getsg
  }%
}
\def\delsavekeys{\XKV@stfalse\XKV@testoptb\XKV@delsavekeys}
\def\gdelsavekeys{\XKV@sttrue\XKV@testoptb\XKV@delsavekeys}
\def\XKV@delsavekeys#1{%
  \XKV@ifundefined{XKV@\XKV@header save}{%
    \XKV@err{no save keys defined for `\XKV@header'}%
  }{%
    \expandafter\XKV@delete\csname XKV@\XKV@header
      save\endcsname{#1}\XKV@getsg
  }%
}
\def\unsavekeys{\XKV@stfalse\XKV@testoptb\XKV@unsavekeys}
\def\gunsavekeys{\XKV@sttrue\XKV@testoptb\XKV@unsavekeys}
\def\XKV@unsavekeys{%
  \XKV@ifundefined{XKV@\XKV@header save}{%
    \XKV@err{no save keys defined for `\XKV@header'}%
  }{%
    \ifXKV@st\expandafter\global\fi\expandafter\let
      \csname XKV@\XKV@header save\endcsname\@undefined
  }%
}
\def\setkeys{\XKV@testopta{\XKV@testoptc\XKV@setkeys}}
\long\def\XKV@setkeys[#1]#2{%
  \XKV@checksanitizea{#2}\XKV@resb
  \let\XKV@naa\@empty
  \XKV@for@o\XKV@resb\XKV@tempa{%
    \expandafter\XKV@g@tkeyname\XKV@tempa=\@nil\XKV@tempa
    \XKV@addtolist@x\XKV@naa\XKV@tempa
  }%
  \ifnum\XKV@depth=\z@\let\XKV@rm\@empty\fi
  \XKV@usepresetkeys{#1}{preseth}%
  \expandafter\XKV@s@tkeys\expandafter{\XKV@resb}{#1}%
  \XKV@usepresetkeys{#1}{presett}%
  \let\CurrentOption\@empty
}
\def\XKV@usepresetkeys#1#2{%
  \XKV@presettrue
  \XKV@for@eo\XKV@fams\XKV@tfam{%
    \XKV@makehd\XKV@tfam
    \XKV@ifundefined{XKV@\XKV@header#2}{}{%
      \XKV@toks\expandafter\expandafter\expandafter
        {\csname XKV@\XKV@header#2\endcsname}%
      \@expandtwoargs\XKV@s@tkeys{\the\XKV@toks}%
        {\XKV@naa\ifx\XKV@naa\@empty\else,\fi#1}%
    }%
  }%
  \XKV@presetfalse
}
\long\def\XKV@s@tkeys#1#2{%
  \XKV@sp@deflist\XKV@na{#2}%
  \XKV@for@n{#1}\CurrentOption{%
    \expandafter\XKV@s@tk@ys\CurrentOption==\@nil
  }%
}
\long\def\XKV@s@tk@ys#1=#2=#3\@nil{%
  \XKV@g@tkeyname#1=\@nil\XKV@tkey
  \expandafter\KV@@sp@def\expandafter\XKV@tkey\expandafter{\XKV@tkey}%
  \ifx\XKV@tkey\@empty
    \XKV@toks{#2}%
    \ifcat$\the\XKV@toks$\else
      \XKV@err{no key specified for value `\the\XKV@toks'}%
    \fi
  \else
    \@expandtwoargs\in@{,\XKV@tkey,}{,\XKV@na,}%
    \ifin@\else
      \XKV@knftrue
      \KV@@sp@def\XKV@tempa{#2}%
      \ifXKV@preset\XKV@s@tk@ys@{#3}\else
        \ifXKV@pl
          \XKV@for@eo\XKV@fams\XKV@tfam{%
            \XKV@makehd\XKV@tfam
            \XKV@s@tk@ys@{#3}%
          }%
        \else
          \XKV@whilist\XKV@fams\XKV@tfam\ifXKV@knf\fi{%
            \XKV@makehd\XKV@tfam
            \XKV@s@tk@ys@{#3}%
          }%
        \fi
      \fi
      \ifXKV@knf
        \ifXKV@inpox
          \ifx\XKV@doxs\relax
            \ifx\@currext\@clsextension\else
              \let\CurrentOption\XKV@tkey\@unknownoptionerror
            \fi
          \else\XKV@doxs\fi
        \else
          \ifXKV@st
            \XKV@addtolist@o\XKV@rm\CurrentOption
          \else
            \XKV@err{`\XKV@tkey' undefined in families `\XKV@fams'}%
          \fi
        \fi
      \else
        \ifXKV@inpox\ifx\XKV@testclass\XKV@documentclass
          \expandafter\XKV@useoption\expandafter{\CurrentOption}%
        \fi\fi
      \fi
    \fi
  \fi
}
\def\XKV@s@tk@ys@#1{%
  \XKV@ifundefined{\XKV@header\XKV@tkey}{}{%
    \XKV@knffalse
    \XKV@ifundefined{XKV@\XKV@header save}{}{%
      \expandafter\XKV@testsavekey\csname XKV@\XKV@header
        save\endcsname\XKV@tkey
    }%
    \ifXKV@rkv
      \ifXKV@sg\expandafter\global\fi\expandafter\let
        \csname XKV@\XKV@header\XKV@tkey @value\endcsname\XKV@tempa
    \fi
    \expandafter\XKV@replacepointers\expandafter{\XKV@tempa}%
    \ifx\@empty#1\@empty\XKV@afterelsefi
      \XKV@ifundefined{\XKV@header\XKV@tkey @default}{%
        \XKV@err{no value specified for key `\XKV@tkey'}%
      }{%
        \expandafter\expandafter\expandafter\XKV@default
          \csname\XKV@header\XKV@tkey @default\endcsname\@nil
      }%
    \else\XKV@afterfi
      \XKV@srstate{@\romannumeral\XKV@depth}{}%
      \csname\XKV@header\XKV@tkey\expandafter
        \endcsname\expandafter{\XKV@tempa}\relax
      \XKV@srstate{}{@\romannumeral\XKV@depth}%
    \fi
  }%
}
\def\XKV@testsavekey#1#2{%
  \ifXKV@rkv\else
    \XKV@for@o#1\XKV@resa{%
      \expandafter\XKV@ifcmd\expandafter{\XKV@resa}\global\XKV@resa{%
        \ifx#2\XKV@resa
          \XKV@rkvtrue\XKV@sgtrue
        \fi
      }{%
        \ifx#2\XKV@resa
          \XKV@rkvtrue\XKV@sgfalse
        \fi
      }%
    }%
  \fi
}
\long\def\XKV@replacepointers#1{%
  \let\XKV@tempa\@empty
  \let\XKV@resa\@empty
  \XKV@r@placepointers#1\usevalue\@nil
}
\long\def\XKV@r@placepointers#1\usevalue#2{%
  \XKV@addtomacro@n\XKV@tempa{#1}%
  \def\XKV@tempb{#2}%
  \ifx\XKV@tempb\@nnil\else\XKV@afterfi
    \XKV@ifundefined{XKV@\XKV@header#2@value}{%
      \XKV@err{no value recorded for key `#2'; ignored}%
      \XKV@r@placepointers
    }{%
      \@expandtwoargs\in@{,#2,}{,\XKV@resa,}%
      \ifin@\XKV@afterelsefi
        \XKV@err{back linking pointers; pointer replacement canceled}%
      \else\XKV@afterfi
        \XKV@addtolist@x\XKV@resa{#2}%
        \expandafter\expandafter\expandafter\XKV@r@placepointers
          \csname XKV@\XKV@header#2@value\endcsname
      \fi
    }%
  \fi
}
\def\XKV@default#1#2\@nil{%
  \expandafter\edef\expandafter\XKV@tempa
    \expandafter{\expandafter\@gobble\string#1}%
  \edef\XKV@tempb{\XKV@header\XKV@tkey}%
  \@onelevel@sanitize\XKV@tempb
  \ifx\XKV@tempa\XKV@tempb
    \begingroup
      \expandafter\def\csname\XKV@header\XKV@tkey\endcsname##1{%
        \gdef\XKV@tempa{##1}%
      }%
      \csname\XKV@header\XKV@tkey @default\endcsname
    \endgroup
    \XKV@ifundefined{XKV@\XKV@header save}{}{%
      \expandafter\XKV@testsavekey\csname XKV@\XKV@header
        save\endcsname\XKV@tkey
    }%
    \ifXKV@rkv
      \ifXKV@sg\expandafter\global\fi\expandafter\let
        \csname XKV@\XKV@header\XKV@tkey @value\endcsname\XKV@tempa
    \fi
    \expandafter\XKV@replacepointers\expandafter
      {\XKV@tempa}\XKV@afterelsefi
    \XKV@srstate{@\romannumeral\XKV@depth}{}%
    \expandafter#1\expandafter{\XKV@tempa}\relax
    \XKV@srstate{}{@\romannumeral\XKV@depth}%
  \else\XKV@afterfi
    \XKV@srstate{@\romannumeral\XKV@depth}{}%
    \csname\XKV@header\XKV@tkey @default\endcsname\relax
    \XKV@srstate{}{@\romannumeral\XKV@depth}%
  \fi
}
\def\setrmkeys{\XKV@testopta{\XKV@testoptc\XKV@setrmkeys}}
\def\XKV@setrmkeys[#1]{%
  \def\XKV@tempa{\XKV@setkeys[#1]}%
  \expandafter\XKV@tempa\expandafter{\XKV@rm}%
}
\XKVcatcodes
\endinput
%%
%% End of file `xkeyval.tex'.

